Federated Learning for Misbehaviour Detection with Variational Autoencoders and Gaussian Mixture Models

Federated Learning (FL) has become an attractive approach to collaboratively train Machine Learning (ML) models while data sources' privacy is still preserved. However, most of existing FL approaches are based on supervised techniques, which could require resource-intensive activities and human intervention to obtain labelled datasets. Furthermore, in the scope of cyberattack detection, such techniques are not able to identify previously unknown threats. In this direction, this work proposes a novel unsupervised FL approach for the identification of potential misbehavior in vehicular environments. We leverage the computing capabilities of public cloud services for model aggregation purposes, and also as a central repository of misbehavior events, enabling cross-vehicle learning and collective defense strategies. Our solution integrates the use of Gaussian Mixture Models (GMM) and Variational Autoencoders (VAE) on the VeReMi dataset in a federated environment, where each vehicle is intended to train only with its own data. Furthermore, we use Restricted Boltzmann Machines (RBM) for pre-training purposes, and Fedplus as aggregation function to enhance model's convergence. Our approach provides better performance (more than 80 percent) compared to recent proposals, which are usually based on supervised techniques and artificial divisions of the VeReMi dataset.

==> Evaluation.tex <==
\section{Evaluation}\label{sec:Evaluation}
For the evaluation of our FL-enabled misbehaviour detection approach, we considered several federated scenarios running in a virtual machine with processor Intel(R) Xeon(R) Silver 4214R CPU @ 2.40GHz with 24 cores and 196 GB of RAM. Furthermore, we use Flower \cite{flower} as the Federated Learning framework. Flower provides an end-to-end implementation and  the possibility to customise several aspects of the model for performing a further evaluation. All the parameters related to our federated scenarios are summarised in Table \ref{tab:summary_fl}. The code and the dataset used are provided in a online repository\footnote{\url{https://github.com/Enrique-Marmol/Federated-Learning-for-Misbehaviour-Detection-with-Variational-Autoencoder-and-Gaussian-Mixture-Mode}}.

\begin{table}[]
\centering
\begin{tabular}{ll}
\hline
\textbf{Framework} & Flower            \\ \hline
\textbf{Model}     & VAE / AE \\ \hline
\textbf{Aggregation function}     & Fed+ \\ \hline
\textbf{Clients}   & From Fig. \ref{fig:value_counts}         \\ \hline
\textbf{Rounds}    & 30                \\ \hline
\textbf{Epochs}    & 1                 \\ \hline
\end{tabular}
\caption{Summary of parameter of our federated scenarios.}
\label{tab:summary_fl}
\end{table}

%\subsection{Dataset description and preprocesing}



\iffalse
\begin{table}[]
\begin{tabular}{llllll}
\centering
\textbf{Attack type:} & \textbf{Description:} &  &  &  &  \\ \cline{1-2}
1: Constant & Vehicle transmits a fixed position &  &  &  &  \\ \cline{1-2}
2: Constant Offset & \begin{tabular}[c]{@{}l@{}}Offset added to vehicle’s actual\\ position\end{tabular} &  &  &  &  \\ \cline{1-2}
3: Random & \begin{tabular}[c]{@{}l@{}}Transmits random position from \\ simulation area\end{tabular} &  &  &  &  \\ \cline{1-2}
4: Random Offset & \begin{tabular}[c]{@{}l@{}}Random position from preconfigured \\ rectangular area around the vehicle\end{tabular} &  &  &  &  \\ \cline{1-2}
5: Eventual Stop & \begin{tabular}[c]{@{}l@{}}Attacker behaves normally for\\ some time and then transmits \\ current position repeatedly\end{tabular} &  &  &  &  \\ \cline{1-2}
\end{tabular}
\caption{Different attacks in VeReMi}
\label{tab:veremi_attacks}
\end{table}
\fi




\subsection{Client division}
%As stated in previous sections, the neural network's input size depends of the histograms dimension,
GMMs require the user to specify the number of components (clusters) before training the model and also, the input size of the neural network, which is the next step, depends on such a number. Instead of selecting a fixed number of components for all the clients, we compute the optimal number of components for each client using silhouette analysis as stated in Section \ref{sec:System}, and consequently, the clients are grouped based on their optimal number of components since different networks with different input sizes will be created (one per group). Fig. \ref{fig:value_counts} shows the number of clients/cars that resulted in having a certain number of components as optimal. As we can see, the most common number of components was 300.
%distribution of the clients in each of the clusters. 
Hence, we will have as many federated scenarios as groups of cars are created based on their optimal number of components.
\begin{figure} [!ht]
	\centering
		\includegraphics[width=\columnwidth]{Images/Evaluation/value_counts.pdf}
	\caption{Number of clients per cluster depending on the number of components}
	\label{fig:value_counts}
\end{figure}

Firstly, we will provide extensive analysis for the group of clients whose optimal number of GMM components is 298. The analysis will be the same for each group of clients that have the same number of components. In that sense, in order not to repeat the process 104 times, as it is the number of groups we encountered, we will secondly provide the final results for the rest of the groups which contain more than 5 clients. The reason for choosing this grouping is to display a better picture comparing all clients' performance. Although the group with 298 components has a fewer number of clients compared to the clusters of 300 and 299 components (20, 93, and 45 clients respectively), the average sample size of the clients is similar between those groups (20453,  19983, and 21004 respectively) and also for the standard deviation (7677, 9760, and 10885), so the clients of this particular case have a similar distribution and therefore having fewer clients can ease results' interpretation and plotting. We will refer in this section to the part of the algorithm that uses either VAE or AE. This analysis includes a comparison of the performance of the autoencoder part depending on the learning rate (\textit{lr}) using the VAE or the AE, the corresponding total metrics (joining GMM and the autoencoder part) of the best case, and the accuracy of the clients' autoencoder part between the best.  

Both VAE and AE are built as equally as possible to ease their comparison. The input layer has the size of the number of GMM components. Next, in the encoder, the first hidden layer has half the size of the input layer, and then the latent space of the AE and the sample layer of the VAE account for a third of the size of the input layer. Finally, the decoder has two layers, the first with half of the size of the input layer,  and the output layer has the size of the input layer. All these layers use ReLU as the activation function except the last one which is the sigmoid function and both use RMSprop as the optimizer. For the rest of the clusters, we compare the results of using AE and VAE with the best \textit{lr}. 
%The selection of the cluster of 298 has been made since it involves a significant quantity of clients, and comparing with the cluster of 300 components (93 clients), and 299 (45 clients) they have a similar size average  of the clients (20453,  19983, and 21004 respectively) and standard deviation (7677, 9760, and 10885), but the case with 298 components consume less than half of time comparing with the others (poner tiempo luego). For all clusters that have more than 5 clients, which are 20 clusters, we have also computed the total accuracy of the system and the accuracy of the autoencoder part using the SAE or VAE, that is the federated part.


\subsection{Particular case analysis: Clients with 298 components}
Looking at Fig. \ref{fig:value_counts}, 20 clients have been grouped with 298 components. In this section, we will analyse the use of the VAE and the AE not only in the federated scenario but also in its distributed counterpart (without using FL). In this part, we differentiate two different types of accuracy. Firstly, the accuracy of the general model, i.e., the accuracy reached with the use of the GMM and the autoencoder part (total accuracy), and the accuracy of only the autoencoder part, since the autoencoder part is the only part that benefits from the FL properties, the GMM part it is the nearly the same every round.

Table \ref{tab:acc_lr} shows the different accuracies of the autoencoder part using different \textit{lr}. Looking at the table we notice that all accuracies for the different \textit{lr} are quite similar, except in the case when $lr=0.05$. In that sense, the VAE gets better performance than the AE using FL, and the distributed scenarios for any \textit{lr}. In this case, the federated VAE reaches a 0.972 of accuracy, whereas the distributed VAE, federated AE, and distributed AE reach 0.928 (\textit{lr} = 0.001), 0.923 (\textit{lr} = 0.005), and 0.936 (\textit{lr}= 0.005) respectively. Comparing the results of the best VAE with the best case of the federated AE in Fig. \ref{fig:comp_client} the variational version shows a better performance in almost all clients.


\begin{table*}[]
\centering
\begin{tabular}{lllll}
\textbf{Learning rate} & \textbf{Federated VAE} & \textbf{Distributed VAE} & \textbf{Federated AE} & \textbf{Distributed AE} \\ \hline
0.001                  & 0.920                & \textbf{0.928}                  & 0.90             & 0.921                  \\ \hline
0.005                  & 0.892                & 0.915                   & \textbf{0.923}      & \textbf{0.936 }                  \\ \hline
0.01                   & 0.767                & 0.792                   & 0.893               & 0.911                  \\ \hline
0.05                   & \textbf{0.972}       & 0.853                   & 0.455               & 0.3640                  \\ \hline
0.1                    & 0.953                & 0.901                   & 0.457               & 0.447                  \\ \hline
\end{tabular}
\caption{Accuracy of different methods varying the \textit{lr}}
\label{tab:acc_lr}
\end{table*}

\begin{figure} [!ht]
	\centering
		\includegraphics[width=\columnwidth]{Images/Evaluation/comparacion_clients_VAE_AEbis.pdf}
	\caption{Comparison of accuracies of autoencoder part between best case of VAE ($lr=0.05$) and AE ($lr=0.005$)}
	\label{fig:comp_client}
\end{figure}

Having set the best \textit{lr} for the VAE, Fig \ref{fig:metrics_GMMVAE} shows the final metrics of the general model, joining the GMM with the VAE. The accuracy of the model is 0.824, end the recall, precision, and f1-score are 0.968, 0.672, and 0.775 respectively. In order to justify the grid chosen in section \ref{sec:System}, Table \ref{tab:timeComparison} provides a comparison of the time consumed by the principal parts of our method that depends on the number of components of the GMM, and the accuracy achieved. In the table, as expected, as the number of components increases, the time involved is higher, especially because of the silhouette analysis. Nevertheless, although the accuracy also increases, the increase of each step is getting lower, from 0.62 to 0.824. Hence, we have set the maximum number of components of the grid at 300, since a wider range will consume an enormous amount of time for an insignificant improvement in accuracy. 

%In order to complete the results of Table \ref{tab:timeComparison}, we obtain that making the grid with 300 components gives 0.824 of accuracy,  with 200 components 0.783, with 100 components 0.705, and with 10 0.62. Hence, a grid with more components will have slowed the process enormously with a insignificant upgrade in the accuracy. 

\begin{table}[]
\begin{tabular}{l|llll}
\textbf{Number of components} & \textbf{10} & \textbf{100} & \textbf{200} & \textbf{300} \\ \hline
\textbf{Silhouette analysis}  & 947         & 21357        & 54298        & 110132       \\ \hline
\textbf{Training GMM}         & 15          & 50           & 202          & 236          \\ \hline
\textbf{Training RBM}          & 28          & 286          & 1028         & 2122 \\ \hline
\textbf{Accuracy}          & 0.62          & 0.705          & 0.783         & 0.824 \\ \hline
\end{tabular}
\caption{Time comparison (in seconds) of main parts that uses GMM depending on the number of components, and the respective accuracy}
\label{tab:timeComparison}
\end{table}



\begin{figure} [!ht]
	\centering
		\includegraphics[width=\columnwidth]{Images/Evaluation/metricas_totales_vae005.pdf}
	\caption{Metrics of the federated scenario using GMM and VAE}
	\label{fig:metrics_GMMVAE}
\end{figure}

Finally, we also compare our work with the case where the GMM and histograms are not used, only applying purely the VAE as a baseline, taking directly the benign dataset, and detecting the attacks using the reconstruction error. This method reaches 0.587 of accuracy, supporting in this way the combination of GMM and histograms with the VAE.


\subsection{General case: All clusters with more than 5 clients}
This section shows the results for all clusters (any number of components) that contain 5 or more clients. Fig. \ref{fig:resto_clientes_total} and Fig. \ref{fig:resto_clientes:ae} provide the accuracy of the general model and the autoencoder part respectively, comparing when AE or VAE is used. For each case, we have selected the best \textit{lr}.
%, as well as the comparison using SAE and VAE using the best learning rate for each case. 
In both figures, it is noticed that for almost every cluster the results using the VAE are higher compared to using the AE.


\begin{figure} [!ht]
	\centering
		\includegraphics[width=\columnwidth]{Images/Evaluation/vae_vs_ae_totalbis.pdf}
	\caption{Comparison between total accuracy of AE and VAE}
	\label{fig:resto_clientes_total}
\end{figure}

\begin{figure} [!ht]
	\centering
		\includegraphics[width=\columnwidth]{Images/Evaluation/vae_vs_aebis.pdf}
	\caption{Comparison between accuracy of AE and VAE}
	\label{fig:resto_clientes:ae}
\end{figure}


Finally, let us compare our results using supervised learning for binary classification using the VeReMi dataset. The recent work \cite{moulahi2022privacy} uses several supervised machine learning algorithms (Support Vector Machines, K-Nearest Neighbour, Naïve Bayes, and Random Forest). The method which reaches the highest accuracy is the support vector machine with an accuracy of 0.8245 . Regarding the other metrics, the best model reaches a precision of 0.91, a recall of 0.5, and f1-score of 0.6. Comparing these values with the clusters of Fig. \ref{fig:resto_clientes_total}, on average, we have obtained an accuracy of 0.8207, a precision of 0.66, a recall of 0.96, and f1-score of 0.77. On the whole, we achieve better results, since we got a similar value in accuracy, and a better value in f1-score means that we obtain a better balanced in recall and precision.%This surpasses the accuracy achieved by some clusters in Fig. \ref{fig:resto_clientes_total}.
 Furthermore, \cite{moulahi2022privacy} divides the dataset into five equally balanced clients, whereas our clients are based on the cars in the VeReMi dataset, obtaining an unbalanced dataset, and being closer to a real case scenario. Comparing our work with a neural network using our division of clients, it reaches an accuracy of 0.88, being higher than most of the clusters.  Although the accuracies of the neural network and the one of the previous work are higher, they have a supervised scenario, which means that the dataset requires to be labelled, which in some cases it may be impossible.

%Their method, nearly 0.60 whereas ours get 0.77











 

==> Introduction.tex <==
\section{Introduction}\label{sec:Introduction}


%Jose Luis: aqui meter resultados con secure aggregation \cite{li2021secure}

%Comentar el tema de las autorregressive networks



%Vehicular Ad Hoc Networks (VANETs) applications are based on the frequent exchange of safety messages by vehicles which provides traffic safety and efficiency \cite{ghosh2009distributed}. It also enables route planning, road safety and e-commerce applications \cite{grover2011machine}. VANETs networks have a short life expectancy, since the network topology changes very frequently, as nodes are in constant movement,  it is frequent that vehicles are out of range of each other. Furthermore, density of the network changes over time, e.g., during rush hours \cite{ruj2011data}. Ensuring their security is an essential part, since an attacker could broadcast wrong location information to create fake traffic jams, false alerts, or ghost vehicles \cite{so2018integrating}.

Misbehaviour detection in vehicular data has attracted significant interest in recent years. Nevertheless, most of the proposed approaches use centralized Machine Learning (ML), applied to massive amounts of data from different vehicles \cite{van2018survey}. %, that are the clients in these scenarios. 
This approach requires all the data produced by the vehicles in the network to be clustered in one huge data centre, which not only produces a delay in the entire process but also leads to privacy issues as driver and passenger data can be shared. Some works \cite{zhang2021survey, lyu2020threats, aledhari2020federated} state the importance of protecting the clients' personal information, and the need of finding new methods that ensure it. In that sense, traditional centralized machine learning is unable to support such ubiquitous deployments and applications due to infrastructure shortcomings such as limited communication bandwidth, intermittent network connectivity, and strict delay constraints \cite{lyu2020threats}. These problems have made researchers move toward more decentralized learning frameworks \cite{billah2022systematic}, such as Federated learning (FL). FL was proposed by Google \cite{mcmahan2017communication} as a solution to the previous problems. FL is a type of collaborative machine learning where instead of sending the data to a central server, the different clients train a common model and only send the weights created during the training phase to that server. This way, their personal information is protected because the clients use their data to train a model, and benefit from the training of other clients without sharing any information about their dataset. The server aggregates all the weights using what is called an aggregation function and sends the result to the clients so that they continue their training using the updated information. The aggregation function is responsible for summarising the clients’ weights in the server into new ones that will be sent back to the clients. A commonly used aggregation function is FedAvg \cite{mcmahan2017communication}, which computes the average of the weights. Nevertheless, in real case scenarios, as our case, the dataset distributions are not independent and identically distributed (non-IID), which causes a deterioration in the performance of FedAvg \cite{campos2021evaluating}. For this reason, we have implemented in our work a more robust aggregation function against the previous scenarios called Fed+ (or Fedplus) \cite{yu2020fed+}, which is designed to handle non-IID data distributions since it removes the condition that all parties have to converge to a single central point.  %Although it is possible that some information can be inferred through these weights, recent works such as \cite{li2021secure} protect the weights by secure aggregation techniques, in which the information shared between clients and server are encrypted by the use of public and private keys. In this way, federated learning assures reliable training without compromising the information of the clients.

The current state of the art for detecting anomalies or misbehaviour is based on supervised learning \cite{uprety2021privacy,boualouache2022federated,boualouache2022survey}, e.g., classifiers and regressors. Supervised techniques need labelled datasets in order to train the model. However, the labelling of the samples is a very resource-intensive and time-consuming process. Usually the labelling can only be done manually \cite{karoly2018unsupervised} and sometimes is not even possible. Supervised algorithms require this intervention to create the labels of the input and set the output \cite{saravanan2018state}, %and also a vast number of trainable parameters of such models, 
and also require the training process to have numerous labelled examples to achieve a proper generalization. This leads to a need for a huge computation time for model training. These inconveniences related to the use of labelled data have led to a groundswell of interest in leveraging unsupervised ML methods that utilise unlabeled data \cite{usama2019unsupervised}. Unsupervised learning is used to extract meaningful information on the structure and hierarchies in the data, relying only on the data samples without the need for ground truth files. The extracted knowledge representation can be used as a basis for a deep model that requires fewer labelled examples, as it already has a good understanding of the hidden nature of the data and should be only fine-tuned for the specific task \cite{karoly2018unsupervised}. All these reasons motivate us to implement unsupervised learning in federated scenarios.%Additionally, some unsupervised techniques, such as autoencoders, need fewer data than other types neural networks for supervised techniques in order to achieve good results \cite{andresini2021autoencoder,chen2018subspace}. This latter fits perfectly in the context of FL, as total data is spread through several clients, relaxing the condition that each client has a huge dataset. All these reasons motivate us to implement unsupervised learning in federated scenarios.



%These reasons motivate us for applying unsupervised learning techniques, which in the context of federate learning has great synergy since some types of techniques need less data in order to perform great results \cite{andresini2021autoencoder,cheng2018deep}. Hence, as data is spread through several clients, it does not need that each client holds a huge amount of data.   

%does not need labelled data. Although supervised algorithms are simpler than unsupervised ones, unsupervised learning can see patterns which in other ways could be difficult to realise. 

%We proposed our work in the context of Vehicular Ad Hoc Networks (VANETs). VANETs applications are based on the frequent exchange of safety messages by vehicles which provides traffic safety and efficiency \cite{ghosh2009distributed}. It also enables route planning, road safety and e-commerce applications \cite{grover2011machine}. VANETs networks have a short life expectancy, since the network topology changes very frequently, as nodes are in constant movement,  it is frequent that vehicles are out of range of each other. Furthermore, the density of the network changes over time, e.g., during rush hours \cite{ruj2011data}. Hence, ensuring their security is an essential part, since an attacker could broadcast wrong location information to create fake traffic jams, false alerts, or ghost vehicles \cite{so2018integrating}.

Our work proposes a combination of clustering techniques and a special case of neural networks called autoencoders for misbehaviour detection. %, which can detect anomalous samples without the data has to be labelled during the training. Clustering techniques are utilised for finding anomalies in unlabeled data. 
Clustering algorithms aim to separate the given unlabelled data into clusters that achieve high inner similarity and outer dissimilarity, without relying on signatures or explicit descriptions of attack classes. %, or labelled data for training. 
%Clustering has attracted interest from researchers in the field of intrusion detection since they allow finding anomalies in unlabeled data without explicit labels \cite{syarif2012unsupervised}. 
In particular, we choose Gaussian mixture models (GMM) as clustering technique since it adds probabilities therefore removing the restriction that one point has to belong only to one cluster. Additionally, GMM-based clustering also performs better in several scenarios where other clustering methods are bound to fail \cite{vashishth2019gmmr}. As mentioned, we use autoencoders, in particular Variational Autoencoders (VAE). The main goal of an autoencoder is to reconstruct the input data passed to the neural network. Since they achieve great success in generating abstract features of high-dimensional data, the detection of abnormal samples increases significantly \cite{said2020network}. %A very important fact is that, as a neural network, autoencoders generate weights during their training part, which can be used in FL. Also, as explained before, autoencoders are lighter and need fewer training samples than others neural networks such as Multi-Layer Perceptons \cite{ramchoun2016multilayer}. 
This combination of these unsupervised approaches such as neural networks and clustering techniques has been reported to be more efficient in anomaly detection \cite{aneetha2012combined}. Additionally, we implement Restricted Boltzmann Machines (RBM), a type of neural network which creates adequate initial weights for the VAE, assuring that no client will get stuck in their training. This method, to the best of our knowledge, has not been used before. We provide a comparison between the performance of the variational and the simple autoencoder (SAE). Our contributions can be summarised as follows:

%Our method works as follows. First, with GMM we divide the clients’ benign dataset into a certain number of groups depending on certain parameters of the GMM, and cluster these clients based on these parameters chosen in their respective GMM. Next, for each cluster, we make a federated environment where the trained model is a combination of GMM and variational autoencoders (VAE), which are a type of autoencoder that mixes probabilities and neural networks. Additionally, we implement Restricted Boltzmann Machines (RBM), a type of neural network which creates adequate initial weights for the VAE, assuring that no client will get stuck in their training. This method, to the best of our knowledge, has not been used before. We also provide a comparison between the performance of the variational and the simple autoencoder (SAE). Our contributions can be summarised as follows:

\begin{itemize}
    \item Creation of a realistic unsupervised misbehaviour detection scenario which implements GMM and VAE using a more sophisticated aggregation function in order to overcome non-iid scenarios.
    %\item Reduction of bandwidth communication by clustering the clients by their number of GMM components.
    \item Overcoming some non-iid issues by the use of RBM.
    \item Improving of results comparing to supervised and unsupervised works using our dataset.

\end{itemize}


The structure of the paper it is as follows:
Section \ref{sec:Preeliminaries} provides a explanation of the concepts used in this paper. Section \ref{sec:Related} analyse other works which use GMM and autoencoders, and autoencoders with FL. Then, in \ref{sec:System} we give a deep description of our misbehavior detection system. Section \ref{sec:Evaluation} describes the results of our solution and compare with other methods, and Section \ref{sec:Conlutions} concludes the paper.

==> Preeliminaries.tex <==
\section{Preliminaries}\label{sec:Preeliminaries}
In this section, we describe the FL and the models involved in our method, that are GMMs, RBMs, autoencoders and their variational version. %We will also describe RBMs that improve autoencoders' performance and have a synergy with federated learning.

\subsection{Federated learning and the aggregation function}
%Federated learning was proposed in \cite{mcmahan2017communication} as an decentralised method to train a machine learning model. 

Nowadays, cyberattacks are getting increasingly more sophisticated, which leads to the need of new datasets to face them. Nevertheless, privacy is becoming a more relevant issue currently, which makes the creation of new datasets in a centralized way difficult adding to other reasons such as the lack of sufficient network connectivity, or policy/regulatory restrictions which prevent free unfettered movement of data \cite{verma2019approaches}.  %with new attacks more difficult to create since it involves the cooperation of several entities in joining their data.
For overcoming this, McMahan proposed in \cite{mcmahan2017communication} FL. FL is a decentralised method which can train a machine learning model ensuring that personal data will not be leaked. 

FL is composed of 2 parts, the central entity (or server), and the data owners (or clients). The communication between these parts is essential for the correct creation of the model. The key of FL is that the clients instead of sharing their own data, they create a model that is trained with their own data and then share the weights of the model. The complete FL scheme is summarised by the following steps:

\begin{itemize}
    \item \textbf{Step 1:} The server initialises the weights of the model and sends them to the clients. 
    \item \textbf{Step 2:} The clients receive the weights and train the model with the number of epochs settled using their own data.
    \item \textbf{Step 3:} The clients send the resulting weights to the server.
    \item \textbf{Step 4:} The server receives, aggregates and sends the weights back to the clients.
    \item \textbf{Step 5:} Steps 2, 3, and 4 are repeated as many times as desired. These repetitions are named \textit{rounds}. 
\end{itemize}


 \begin{figure} [!ht]
	\centering
		\includegraphics[scale=0.2]{Images/Preeliminaries/fl_scheme_ae.pdf}
	\caption{Pictorial description of FL. First the clients train their models that round (1) and send the resulting weights to the server (2). Next, the server aggregates those weights (3) and send them to the clients (4). Finally, the clients start the training again.}
	\label{fig:FLscheme}
\end{figure}

A visual description of the model is displayed in Fig. \ref{fig:FLscheme}. In the picture, in (1) the clients train the model using their dataset. Next, in (2), they send their weights to the server. In (3), the server aggregates all the weights into new ones using the corresponding aggregation function. Finally, in (4) the server sends the aggregated weights to the clients, which start again with (1). For aggregating the weights in the server, we used Fed+ \cite{yu2020fed+} since, as explained in section \ref{sec:Introduction}, it can handle better non-IID scenarios \cite{campos2021evaluating}. The main characteristic of Fed+ is that parties are not forced to converge to a single central point, as explained below. Hence, the weights are uploaded following the following equation:
 \begin{equation} \label{eq:Fed+weights}
    W^{k+1} = \theta[W^k - \nu \nabla f_k(W^k)] + (1-\theta)Z^k,
\end{equation}
where $\nu$ is the learning rate, $\theta = \frac{1}{1+\nu\mu}$ is a constant that controls the degree of regularisation, and $Z^k$ is the average of clients' weights. As the new weights are an average of local weights and global weights, this means that each party has different weights does not depend on the fact that all clients converge to the same point.




\iffalse %Comentado
The process of aggregation can be done by using different functions. As explained in section \ref{sec:Introduction} FedAvg \cite{mcmahan2017communication} is the most common one, it computes the average of the weights, as represented in the following formula:
 $$W = \sum_K \frac{D_k}{D}W^k,$$
 where $W_k$ are client $k$ weights, $D_k$ is client $k$ data length, $D$ is the total data length, and $W$ are the weights which are passed to the clients. As explained previously in section \ref{sec:Introduction}, the performance of FedAvg can be deteriorated when the clients' datasets are non-IID \cite{campos2021evaluating}. For that reason, we use Fed+ \cite{yu2020fed+} (or Fedplus). The main characteristic of Fed+ is that parties are not forced to converge to a single central point, as explained below. Hence, the weights are uploaded following the following equation:
 \begin{equation} \label{eq:Fed+weights}
    W^{k+1} = \theta[W^k - \nu \nabla f_k(W^k)] + (1-\theta)Z^k,
\end{equation}
where $\nu$ is the learning rate, $\theta = \frac{1}{1+\nu\mu}$ is a constant that controls the degree of regularisation, and $Z^k$ is the result of $B(W^k,\Tilde{W})$. As the new weights are an average of local weights and global weights, this means that each party has different weights does not depend on the fact that all clients converge to the same point.
 

Firstly, in FedAvg the objective function is 
\begin{equation} \label{eq:Fed+1}
    \text{min }F(W) = \frac{1}{D}\sum f_k(W^k) \text{ subject to } w_i = w_i^k,
\end{equation}
where $f_k$ is the loss function of client $k$. In the case of Fed+, the idea is to add a penalty function to replace the hard condition of Eq. \ref{eq:Fed+1} which requires all weights converge to the same point. Hence, the new equation will be:
\begin{equation} \label{eq:Fed+2}
    \text{min }F_\mu(W) = \frac{1}{D}\sum [f_k(W^k) +\mu B(W^k,A(W))], 
\end{equation}
where $\mu>0$ is a penalty constant, $A$ is an aggregation function of the clients' weights, and $B(\cdot,\cdot)$ is a distance function that penalises the deviation of
a local model $W^k$ from the output of $A(\cdot)$. 

Hence, applying this to the local weights, the weights are updated by the formula 
\begin{equation} \label{eq:Fed+weights}
    W^{k+1} = \theta[W^k - \nu \nabla f_k(W^k)] + (1-\theta)Z^k,
\end{equation}
where $\nu$ is the learning rate, $\theta = \frac{1}{1+\nu\mu}$ is a constant that controls the degree of regularisation, and $Z^k$ is the result of $B(W^k,\Tilde{W})$. This equation means that the model of each party does not depend on the fact that all weights converge to the same point.
\fi


\subsection{Gaussian mixture models}
A GMM is a probabilistic model that assumes all the data points are generated from a mixture of a finite number of Gaussian distributions with unknown parameters. Formally, a GMM of $K$ components is a parametric probability density function represented as a weighted sum of $K$ normal distributions, i.e.:
$$p(x|\mu_1,\dots,\mu_K,\sigma_1,\dots,\sigma_K,\pi_1,\dots,\pi_K)=\sum_K \pi_i \mathcal{N}(\mu_i,\sigma_i)$$

where $\mu_i$ are the means, $\sigma_i$ the variances, $\pi_i$ the proportions weights (which sum one and are positives), and \mathcal{N} is a  Gaussian with specified mean and variance. The purpose of using GMMs is the division of the dataset observations into $K$ groups or clusters. Due to their probabilistic nature, GMMs differ from other clustering methods such as K-means \cite{awasthi2012improved} in the fact that an observation can belong to more than one cluster. More specifically, GMMs estimate the likelihood of every observation belonging to each component, and assign the observation to the most likely one. In our work, we exploit these probabilities to classify samples as anomalous or not anomalous. Additionally, GMM presents other advantages such as adapting to the shape of the clusters, handling missing data, and taking into account the variance of the data. These properties are described in depth in  \cite{reynolds2009gaussian}.


\iffalse
\subsection{Autoencoders}
An autoencoder is a particular case of neural network where the input and output dimensions coincide \cite{bishop1994neural}. Indeed, autoencoders are a unsupervised learning technique, which enables us to train the model without using labelled data. Autoencoders consist of 2 parts, an encoder and a decoder which are symmetric, i. e., the decoder has the same number of hidden layers as the encoder but backwards, which is shown in Fig. \ref{fig:autoencoderImage}. The encoder takes the input data and compresses it through the hidden layers into a lower dimension code, called \textit{latent space} ($Z$). Then, the decoder reconstructs this latent space into its original state, that is the input data. This reconstructed data will not be exactly equal as it was at the beginning, i. e., the output will not be an exact copy as the input. However, the main objective of the autoencoder is to minimize this difference, called reconstruction error, that is computed as the Root Mean Square Error (RMSE) between the input ($X$) and the output ($\hat{X}$) data.

\begin{equation}
    Reconstruction\, error = ||X - \hat{X}||= \sqrt{\frac{1}{n}\sum{(x_i - \hat{x}_i})}
    \label{eq:RE}
\end{equation}

One of the characteristics of the autoencoders is that they reconstruct data accurately if they are trained with data of the same type, in our case benign data. Other types of data will have high reconstruction errors. This enables us to train the model with only benign data, and use it to detect anomalies. For deciding which samples are benign and which not, the user selects an arbitrary threshold after the training phase, and then, if the difference between a sample and its copy, i.e., the output of the autoencoder, exceeds that threshold, it will be considered an anomaly. The choice of the threshold is crucial since it must cover almost all of the benign cases and exclude the attacks. The ways for selecting this threshold are varied, in \cite{choi2019unsupervised} they choose the threshold base on the mean and standard deviation of the reconstruction error, \cite{mirza2018computer} and \cite{ko2020adaptable} try different thresholds until getting the best performance. In our case, we have considered a threshold based on the mean and standard deviation of the reconstruction error. This approach will be detailed better in Section \ref{sec:System}.% On the other hand, another reason why we have chosen autoencoders is they need fewer training samples and are computationally lighter than usual neural networks \cite{andresini2021autoencoder,cheng2018deep}. Furthermore, they are part of unsupervised learning techniques, which enables us to train the model without using labelled data.
\fi

\begin{figure} [!ht]
	\centering
		\includegraphics[scale=0.4]{Images/Preeliminaries/Autoencoder.pdf}
	\caption{Pictorial description of an autoencoder. A simmetric fully connected neural network where the input is encoded through the encoder to the latent space to be reconstructed by the decoder.}
	\label{fig:autoencoderImage}
\end{figure}

\subsection{Variational autoencoders}

An autoencoder \cite{bishop1994neural} is a particular case of neural network. where the input and output dimensions coincide, and its layer structure is symmetric. Autoencoders consist of an encoder, and a decoder, as can be seen in Fig. \ref{fig:autoencoderImage}. The encoder takes the input data and compresses it through the hidden layers into a lower dimension code, called \textit{latent space} ($Z$). Then, the decoder reconstructs this latent space into its original state, that is the input data. The main goal of autoencoders is to create a copy as close as possible to the original data. The difference between the input and output will be called reconstruction error, and shall be measured using the Root Mean Square Error (RMSE). Autoencoders enable us to train the model with unlabelled data. Training the model with only benign data will produce high reconstruction error when malign data is passed. Hence, a threshold is set to decide which samples are benign or malign.

One of the main characteristics of autoencoders is the latent space $Z$, where all the information is collapsed. VAEs \cite{kingma2013auto} are a kind of autoencoder whose encodings distribution is regularized, i.e., approaches a normal distribution during the training in order to ensure that its latent space has a handful of properties allowing us to generate some new data \cite{zhang2021federated, yao2019unsupervised, sun2018learning, an2015variational}. The main difference between a VAE and a SAE is that the VAE is a stochastic generative model that provides calibrated probabilities, while an SAE is a deterministic discriminative model that does not have a probabilistic foundation. SAEs have issues with generating new samples, which often can make the decoder provide misleading results since all the information condensed in the latent space is disorganised. For that reason, the VAE tries to map the encoder distribution $q(Z|X)$ to a normal distribution for providing more order in the latent space. For this purpose, the \textit{reparameterization trick} is carried out. From this distribution $q(Z|X)$ we take its mean $Z_\mu$ and standard deviation $Z_\sigma$. With these two latent variables, we create a sample a la latent variable $Z$ which will be passed to the decoder in order to create the predicted output $\hat{X}$. This method also ensures that the network can be trained using backpropagation.  %This consists of adding two layers; one is the mean ($Z_\mu$), and the other is the standard deviation ($Z_\sigma$) of the distribution $q(Z|X)$, which creates a new sample in another layer that passes it to the decoder. This is represented in Fig. \ref{fig:VAEimage}




%The latent space in the VAE is composed of 3 layers. First, two parallel layers, one is the mean ($Z_\mu$), and the other is the standard deviation ($Z_\sigma$) of the distribution created by the encoder. The third layer is a vector $Z$ created by the two previous layers which is a sample from a Multi-variate Gaussian model with mean $Z_\mu$, and standard deviation $Z_\sigma$. This new vector is then passed to the decoder and generates the copy of the input. The structure of VAE is reflected in Fig \ref{fig:VAEimage}.

\begin{figure} [!ht]
	\centering
		\includegraphics[scale=0.35]{Images/Preeliminaries/Vae.pdf}
	\caption{Pictorial description of a VAE. Similar to the SAE, but the latent space is change by three layers to ensure the encoder follows a normal distribution.}
	\label{fig:VAEimage}
\end{figure}


Once the VAE has been described, the loss function has to be set.  The main goal of VAE is to create a copy of an input vector. Hence, the RMSE has to be minimized. At the same time, as said previously, the model distribution needs to be as close as possible to a standard gaussian. For this, the Kullback–Leibler Divergence \cite{joyce2011kullback} (KL-divergence) function is used. This function measures how similar two distributions are. Hence, this difference between the encoder distribution and a standard distribution  using the KL-divergence has to be as close as 0 as possible. Therefore, the loss function of VAE is:


\begin{equation}
    Loss(X,\hat{X}) = Loss_{RMSE}(X,\hat{X}) + KL(q(Z|X),\mathcal{N}(0,1))
\end{equation}




%\subsection{Restricted Boltzmann Machines}
%The difficulty of training autoencoders is that the weights often get stuck and do  not converge if they start off in a bad initial state. To address this, Hinton and Salakhutdinov \cite{hinton2006reducing} found that they could use pre-trained RBMs  to create a good initialization state for autoencoders. An RBM is a stochastic neural network model with two-layer structure, symmetric connection and no self feedback, which has full connection between layers and no connection within layers. The first layer is call the visible layer and contains the original input, and the second layer is called the hidden layer. Among their applications we find feature extraction, pattern recognition, dimensionality reduction, data classification, and several others. In this work, as in \cite{wu2021research,pacheco2018restricted,saravanan2020deep}, we use the RBM for pre-training the autoencoder. Solving these RMBs with the shape of the encoder will give us the initial weight of the autoencoder.








 



==> Related_work.tex <==
\section{Related Work}\label{sec:Related}

Even though FL is a relatively novel technique, there exists a plethora of works in supervised misbehaviour detection that use FL. However, unsupervised techniques, such as AE, k-means, or deep belief networks, are still in development in this field. Our technique combines GMM and autoencoders for the purpose of unsupervised misbehaviour detection. This approach is scarce in current literature, and when it is present, it differs from ours as we will explain further. We have divided this section in two parts. First, we describe works that use GMM and AEs in a non federated setting. And second, we have gathered works that use AEs with FL in an unsupervised manner, whether it is variational or not.

%Furthermore, our technique, which combines GMM and autoencoders, described in \ref{sec:System} is also scarce in current literature and differs from ours. 


\subsection{Combination of GMM and autoencoders without FL}
The combination of GMM and AEs is an approach that has not been widely explored so far. A Deep Autoencoding Gaussian Mixture Model (DAGMM) for unsupervised anomaly detection is presented in \cite{zong2018deep}. %Their model utilises a deep autoencoder to generate a low-dimensional representation and reconstruction error for each input data point, which is further fed into a GMM. 
DAGMM consists of a compression network for reducing the dimension of the input samples by a deep AE, and an estimation network which predicts their likelihood/energy in the framework of GMM. First, the deep AE is trained with the data on the compression network. Then, the estimation network is able to make meaningful density estimations.
%the use GMM to classify in different clusters but they did it directly, without histograms.
\cite{an2022ensemble} proposes to use unsupervised ensemble AEs connected to the GMM to adapt to multiple domains regardless of the skewness of each domain. In such work,  ensemble AEs and GMMs are jointly optimized by transforming the optimization of the objective function into a Lagrangian dual problem. Then, they use the Expectation-Maximization (EM) algorithm, which consists of two parts, the ensemble network and the estimation network. Firstly, they use the AE for input dimensionality reduction, and then the estimation network estimates the sample density and classifies those samples with high density as anomalous samples.
%they uses to phases. First the autoencoder part and then pass it to a ensemble model which uses GMM
% variational
Lastly in \cite{liao2018unified}, the authors propose a unified Unsupervised Gaussian Mixture VAE for outlier detection. The VAE first trains a generative distribution and extracts reconstruction-based features. Then they adopt a deep brief network to estimate the component mixture probabilities of the GMM by the latent distribution and extracted features, which is further used by the GMM to estimate sample densities with the EM algorithm.




\subsection{Federated Learning and Autoencoders}

%In \cite{aouedi2022fluids} they make a simple work with a autoencoder and with the dataset UNSW-NB15 
In this section, we focus on the works which combine Federated Learning and AEs, either variational or regular. 
A federated version of the previously described methodology named DAGMM \cite{zong2018deep} is presented in \cite{chen2019network}. They aimed to enhance their model with the federated learning benefits related to the privacy of data of the clients by making each client share its weights of the AE part. \cite{rey2022federated} investigates the possibilities enabled by FL concerning IoT malware detection and studies security issues inherent to this new learning paradigm. In such work, they use both supervised and unsupervised learning.  For the unsupervised method they use AEs for detecting anomalies as usual. That is, training the model with benign data and then classifying those samples with high reconstruction error as malign data.
Other works such us \cite{preuveneers2018chained, cetin2019federated, alazzam2022federated} also incorporate AEs in its federated environment but in other contexts, such as blockchain and wireless networks. All of them, as in the previous work, detect the anomalies by those which surpass the reconstruction error.
%they use the N-BaIoT iot, they use both supervised and unsupervised learning. For the unsupervised learning they use autoencoders. Both works used a direct autoencoder without using GMM, they pass the benign dataset directly.
%\cite{zhao2020semi} uses autoencoders in an FL setting for activity recognition
In \cite{wu2022fl}, an anomaly detection classification model that incorporates Federated Learning and mixed Gaussian variational self-encoding networks named MGVN is proposed. The MGVN network model first constructs a variational self-encoder using a mixed Gaussian prior to extract features from the input data, and then it constructs a deep support vector network with the mixed Gaussian variational self-encoder to compress the feature space. They used a convolutional AE whose encoder part is obtained through the mixed Gaussian variational self-encoder, then the anomalous traffic is detected by using a threshold.

Comparing the works of both sections with ours. The usual way the other authors combine the GMM and AEs is by applying first the AE and then passing the results to the GMM. However, we first apply the GMM and transform the data before passing it to the AE as in \cite{zolotukhin2016increasing, garcia2021distributed}, as will be explained in the following section. This method allows us to learn high-level features from low-level ones and formulate proper features for pattern classification, allowing the model to generate more abstract features that are invariant to local changes of the input. In \cite{wu2022fl}, they also start applying the GMM part, but they do not transform the AE's input data.


==> System_Model.tex <==
\section{System model}\label{sec:System}
In this section, we describe the dataset that will be used to evaluate our methodology and its preprocessing. Next, we describe all the parts involving our misbehaviour detection system.

\subsection{Dataset and preprocessing}
In this work, we have used the previously existing VeReMi dataset \cite{so2018integrating} which is a simulated dataset that was created using VEINS and the Luxembourg SUMO Traffic (LuST) scenario \cite{7385539}. The LuST scenario is a traffic simulation scenario validated with real driving data. VeReMi utilizes a subsection of the LuST scenario. For creating the dataset they simulate 225 scenarios considering 5 position forging attacks, 3 vehicle densities (low, medium and high), 3 attacker densities (10, 20 and 30 percent), and each parameter set was repeated 5 times for randomization. Finally the dataset contains the log messages of almost 500 vehicles. Each file maintains a record of BSMs received by a single vehicle (same ID) from neighbouring vehicles (300-meter range) during its entire journey. The files are converted to CSV files differentiating between benign and malign samples. %labeling the type of attack, which are reflected in table \ref{tab:veremi_attacks}, being type 0 benign traffic

Once the dataset is chosen, we have to preprocess it since our prior works proved that using such a dataset directly can lead to undesirable results \cite{campos2021evaluating}. Firstly, we use SMOTE-Tomek \cite{batista2003balancing}, a combination of oversampling and undersampling techniques in order to balance the class ratio. The new samples in the dataset are created through SMOTE technique by making linear combinations between close points of the less represented class. Then, Tomek Links is in charge of removing neighbour points that belong to different classes in order to make the classes more differentiable. Initially, the balance of the clients dataset is 75\% benign 25\% malign. After applying SMOTE-Tomek, the balance is nearly 50-50 in all clients.

\subsection{Detection system}
\subsubsection{Description of the scenario}
The overall system model of our misbehaviour detection approach consists of several vehicles equipped with a ML module to perform the local training. This module trains a local ML model on each vehicle's data and the messages among themselves and the received ones by other vehicles by BSM messages to update the global model shared by the server node in each training round. In case of detecting a misbehaviour, they can communicate such information to the server, which will store the new data in the database. For the communication with the server, vehicles’ messages go through road ITS stations. First, to communicate with these road ITS stations, wireless links are used and then, the communication between the road ITS stations and the cloud is mostly fixed. Based on the previous description, in this system model, vehicles act as FL clients performing local training by using the VeReMi dataset \cite{so2018integrating} (see Section \ref{sec:Evaluation}) and the global model, which is shared by the server in each training round. The server implements an aggregation method (as described in Section \ref{sec:Preeliminaries}) to aggregate the local results from the FL clients. The resulting aggregated model is sent again to the FL clients to be updated through a new training round. 

\subsubsection{Overview of the system}
A global overview of our system model can be looked at Fig. \ref{fig:systemModel}, where the interaction of all the steps involved is reflected. Our model will consist of 3 parts. Firstly, before applying the FL, the clients train the GMM and then make the histograms that will be the dataset used in the VAE (1). Furthermore, the initial weights of the RBMs are created in this step using these histograms (these two steps will be explained deeply in the next section).  Next is the FL part, where after the initialization, the clients form a federated environment to train their VAE models using the histograms created. Finally, the third part is the local misbehaviour detection (3). After the FL part, each client uses the model created to classify the samples into benign and malign samples. First, the samples pass an initial filter using the GMM created in part (1) to classify the samples which can be labelled easily. Then for the rest of the samples, their histograms will be created and the VAE will calculate their reconstruction error and check whether is higher or lower than the threshold set after part (2). % we have the local misbehaviour detection (part (2)), in which malign samples are detected in each client, they apply the GMM as a first filter to classify the samples. For the rest of samples, with the VAE model trained by FL previously, they classify the remaining samples based on the threshold set and the end of the FL.


\begin{figure*} [!ht]
	\centering
		\includegraphics[scale=0.24]{Images/Detection_Model/esqmod.pdf}
	\caption{Pictorial description of our the detection model. There are three parts, the first one (1), is the initialization, where the clients create the GMM and train it to create the histograms. Also, they use RBM to create the initial weights of the VAE. Then, in (2), clients create a federated environment to train their VAE models. And finally, in (3), the local misbehaviour detection is carried out, where each client classifies the samples as benign or malign using the model trained and the threshold $th$ set.}
	\label{fig:systemModel}
\end{figure*}


\iffalse
\begin{figure*}[!htb]
\centering
  \begin{subfigure}{\columnwidth}
    \includegraphics[width=\linewidth]{esqmod1.pdf}
    \caption{Metrics using the original Veremi dataset with FedAvg (Scenario 1) and Fed+ (Scenario 2)} \label{fig:1a}
  \end{subfigure}%
  \hspace*{\fill}   % maximize separation between the subfigures
  \begin{subfigure}{\columnwidth}
    \includegraphics[width=\columnwidth]{esqmod2.pdf}
    \caption{Metrics using the balanced Veremi dataset with FedAvg (Scenario 3) and Fed+ (Scenario 4)} \label{fig:1b}
  \end{subfigure}%
  \hspace*{\fill}   % maximizeseparation between the subfigures
\caption{Comparison of the different scenarios with the original Veremi dataset and balanced Veremi through SMOTE-Tomek} \label{fig:comparacion_escenarios}
\end{figure*}
\fi

\subsubsection{Model training}
Before classifying the samples, the VAE model has to be trained. First, given a client, we preprocess its dataset as described in section \ref{sec:Evaluation}, and we use the 80\% of the benign dataset to train the GMM with the number of components previously optimised using the Silhouette coefficient \cite{rousseeuw1987silhouettes}, which  is a metric used to calculate the performance of a particular clustering by examining how separated and compact the clusters are. We compute the Silhouette coefficient when partitioning the data from 2 to 300 groups or components. The reason for choosing this range is justified in section \ref{sec:Evaluation}. In summary, a wider range will provide more accurate results, but the trade-off between the performance and the time consumed will be unworthy. This first application of the GMM is only for training the GMM model and separating the benign traffic into several groups which will serve as the first step in order to choose which samples are benign and which are malign.
%In order to make a decision on the range of partitions we wanted to try, we compared the computing time of the different parts of our method that are affected most by the number of components of the GMM in Table  \ref{tab:timeComparison}. As one can anticipate, the table shows exponential growth of time (in seconds) as the number of components increases, joining this with the results of the next section we decided to set 300 as the maximum number of components.

Once the GMM has divided the benign dataset as many groups as components set, to classify a new point we calculate the value of its likelihood function \cite{etz2018introduction}. If this value is greater than 1, it means that it belongs to one of the groups created by the GMM, so it is classified as benign. If it is equal to 0, it does not belong to one of the groups of the GMM, so it is classified as anomalous. Nevertheless, the samples whose value is between 0 and 1 could be attacks that can mirror the normal traffic. For those that are not so clearly discriminated, we applied a technique based on computing histogram vectors \cite{zolotukhin2016increasing}, that is used in previous works \cite{garcia2021distributed}. This technique creates a matrix $H$ which contains the histograms vectors $h^i = (h^i_1,h^i_2,\dots,h^i_K)$, where $K$ is the number of clusters (equal to the number of GMM components) and $h^i_k$ is the number of features of the sample $i$ which are within the cluster $k$. This histogram $H$ will be used as the input data for training the VAE, whose input dimension will be the number of components previously chosen. 

The training of the VAE is the part that will be federated, all the clients will train the VAE sharing the weights produced during the training. After this training, we set the threshold as

\begin{equation}
    th = mean(RE)+0.01*std(RE)
\end{equation}
where $mean(RE)$ and $std(RE)$ are the mean and standard deviation of the reconstruction error respectively. We use this formula since it will give us a value close to the 95-percentile.


One of the drawbacks of the AEs is that the weights during the training often get stuck and do not converge if they start in a bad initial state. Hence, in our case, as there are a high number of clients involved in FL, it is probable that several clients can get stuck and consequently harm the federated environment. To prevent this, we use RBMs, a stochastic neural network that Hinton and Salakhutdinov \cite{hinton2006reducing} found that they could use trained RBMs to create a correct initialization state for AEs. 

An RBM is a stochastic neural network model with a two-layer structure, symmetric connection and no self-feedback, which has a full connection between layers and no connection within layers. The first layer is called the visible layer and contains the original input, and the second layer is called the hidden layer. Among their applications, we find feature extraction, pattern recognition, dimensionality reduction, data classification, and several others. However, as in \cite{wu2021research,pacheco2018restricted,saravanan2020deep}, we will use the RBM for pre-training the VAE, giving us the initial weights for training, assuring its convergence in this case. This pre-training will be made with the same dataset used by the VAE.





\subsubsection{Classifing the samples}
In order to classify the samples as benign or malign, as can be seen in Algorithm \ref{alg:cap}, the GMM makes a first classification, detecting the ones which can be classified easily. In this part, unlike in the training phase, we apply the GMM to a dataset that contains malign and benign traffic. As mentioned in the previous section, we apply the likelihood function associated with the GMM. The ones with a value greater than 1 will be considered benign traffic, and the ones with a value of 0 will be malign traffic.  For those whose likelihood function is between 0 and 1, we transform them into histograms and pass them to the VAE model resulting from the federated training, which will make the final decision based on whether the reconstruction error is higher or not than the threshold previously set. The testing part of our model will be performed by the 20\% of the benign dataset not taken in the training part, with a sample of the same size of malign data. 

\begin{algorithm}
\caption{Our misbehaviour detection system}\label{alg:cap}
\begin{algorithmic}
\REQUIRE $B_k$ Bening dataset of client $k$, $D_k$ Testing dataset of client $k$, $GMM_k$ gaussian mixture model of client $k$, $VAE_k$ VAE model of client $k$
\ENSURE  Accuracy of the model $a$ \\
Train $GMM_k(B_k)$ \\
Create initial weights with $RBM_k$ \\
Create histograms $H_k$ of $B_k$ \\
Train $VAE_k(H_k)$ \\
Set threshold $th$ \\

\FOR{$x\in D_k$}
$p = LF_{GMM_k}(x)$ where $LF_{GMM_k}$ is the likelihood function of $GMM_k$ \hfill \break
\IF{$p\geq 1$} \hfill \break
$x$ is benign
\ELSIF{$p= 0$}
$x$ is anomalous
\ELSE
Create histogram $H$ of $x$ \hfill \break
\IF{$RE(H) > th$} \hfill \break
$x$ is anomalous
\ELSE
$x$ is benign
\ENDIF
\ENDIF
\ENDFOR \\
Calculate confusion matrix $M$.
\end{algorithmic}
\end{algorithm}



==> System_Model_mal.tex <==
\section{Detection system}\label{sec:Systemmal}
Our system for misbehaviour detection is constituted of two parts, the GMM and the VAE. To detect anomalous samples, we train our model with benign traffic, so that when something differs from them, the system identifies it as malign data. 

First, given a client, we preprocess its dataset as described in section \ref{sec:Evaluation}, and we use the 80\% of the benign dataset to train the GMM with the number of components previously optimized using the Silhouette coefficient \cite{rousseeuw1987silhouettes}%\footnote{\url{https://scikit-learn.org/stable/auto_examples/cluster/plot_kmeans_silhouette_analysis.html}}, 
, which  is a metric used to calculate the goodness of a particular clustering by examining how well the clusters are separated and how compact the clusters are. We computed the Silhouette coefficient when partitioning the data from 2 to 300 groups or components. %which measures the distance between the resulting clusters, between 2 and 300 components. 
%A wider range could have provided more accurate results. 
In order to make a decision on the range of partitions we wanted to try, we compared the computing time of the different parts of our method that are affected most by the number of components of the GMM in Table  \ref{tab:timeComparison}. As one can anticipate,
the table shows exponential growth of time (in seconds) as the number of components increases, joining this with the results of the next section we decided to set 300 as the maximum number the components. %so we decided to establish 300 as the maximum number of components that each client could be partitioned into.
%However, if we look at Table \ref{tab:timeComparison}, it gives us a comparison of
Once the GMM has divided the benign dataset as many groups as components set, to classify a new point we calculate the value of its likelihood function \cite{etz2018introduction}. If this value is greater than 1, it means that it belongs to one of the groups created by the GMM, so it is classified as benign. If it is equal to 0, it does not belong to one of the groups of the GMM, so it is classified as anomalous. Nevertheless, the samples whose value is between 0 and 1 can be attacks which can better mirror the normal traffic. For those that are not so clearly discriminated, we applied a technique based on computing histogram vectors \cite{zolotukhin2016increasing}, that is used in previous works \cite{garcia2021distributed}. This technique creates a matrix $H$ which contains the histograms vectors $h^i = (h^i_1,h^i_2,\dots,h^i_K)$, where $K$ is the number of clusters and $h^i_k$ is the number of features of a sample $i$ which are within the cluster $k$. This histogram will be used as the input data for training the autoencoder, whose input dimension will be the number of components previously chosen. After this training, we set the threshold to 

\begin{equation}
    th = mean(RE)+0.01*std(RE)
\end{equation}
where $mean(RE)$ and $std(RE)$ are the mean and standard deviation of the reconstruction error respectively.


\begin{table}[]
\begin{tabular}{l|llll}
\textbf{Number of components} & \textbf{10} & \textbf{100} & \textbf{200} & \textbf{300} \\ \hline
\textbf{Silhouette analysis}  & 947         & 21357        & 54298        & 110132       \\ \hline
\textbf{Training GMM}         & 15          & 50           & 202          & 236          \\ \hline
\textbf{Training RBM}          & 28          & 286          & 1028         & 2122 \\ \hline       
\end{tabular}
\caption{Time comparison (in seconds) of main parts that uses GMM depending on the number of components}
\label{tab:timeComparison}
\end{table}



Hence, the algorithm for classifying a new sample, whose pseudo-code is provided in \ref{alg:cap}, is as follows. Firstly, from the dataset we take the benign samples, and split them into 80\% for training and the other 20\% is joined with a sample of the same size of malign data in order to complete the testing data. We train the GMM model, create the histograms and train the autoencoder model with the training data. Once the training part has finished, we start the testing of the model. For each sample of the testing data, first, its likelihood function is calculated to check whether it belongs or not to one of the clusters. Depending on their value, the ones with a value equal to 0 are classified as attack, since as it was said before, they do not belong to any cluster. The ones with a value greater or equal to 1 belong to some cluster, hence they are classified as benign. For those datapoints whose value is between 0 and 1, we make its histograms and pass them to the autoencoder, and if the reconstruction error is less or equal than the threshold set previously, it is benign, and if it is greater than the threshold, it is an attack.



\begin{algorithm}
\caption{Our misbehaviour detection system}\label{alg:cap}
\begin{algorithmic}
\REQUIRE $B_k$ Bening dataset of client $k$, $D_k$ Testing dataset of client $k$, $GMM_k$ gaussian mixture model of client $k$, $AE_k$ autoencoder model of client $k$
\ENSURE  Accuracy of the model $a$ \\
Train $GMM_k(B_k)$ \\
Create initial weights with $RBM_k$ \\
Train $AE_k(B_k)$ \\
Set threshold $th$ \\

\FOR{$x\in D_k$}
$p = LF_{GMM_k}(x)$ where $LF_{GMM_k}$ is the likelihood function of $GMM_k$ \hfill \break
\IF{$p\geq 1$} \hfill \break
$x$ is benign
\ELSIF{$p= 0$}
$x$ is anomalous
\ELSE
\IF{$RE(x) > th$}
$x$ is anomalous
\ELSE
$x$ is benign
\ENDIF
\ENDIF
\ENDFOR \\
Calculate confusion matrix $M$.
\end{algorithmic}
\end{algorithm}

\begin{figure} [!ht]
	\centering
		\includegraphics[scale=0.5]{Images/Detection Model/esquem modelo.pdf}
	\caption{Pictorial description of our the detection model. First, given a set of samples, the GMM classifies the one which are clearly benign or malign. For those which are in a intermediate point, their histograms are calculate and pass them to the autoencoder, previusly trained with RMBs, to finally classify those samples.}
	\label{fig:systemModel}
\end{figure}

%The model reliability is tested by using as input data a new dataset that contains benign and malign traffic. As said previously, only benign traffic is used for creating the GMM cluster. Then, the 80\% of the samples for making the histograms and then the autoencoder's threshold. The remaining 20\% with a sample of the same size will be used for the testing part. Therefore, we use likelihood function to classify the samples, the ones with value 0 means that it is clearly an attack, they does not belong to any cluster as said before, and the ones with value greater or equal to 1 belong to some cluster, hence they are benign. For those whose value is between 0 and 1, we make the histograms and pass it to the autoencoder, if the reconstruction error is less or equal than the threshold set previously, it is benign, and if it greater than the threshold, it is an attack. 

\iffalse
\begin{figure*} [!ht]
	\centering
		\includegraphics[scale=0.6]{Images/Detection Model/Detection model.drawio.pdf}
	\caption{Pictorial description of of the detection model.}
	\label{fig:systemModel}
\end{figure*}
\fi

==> introduction2.tex <==
\section{Introduction}\label{sec:Introduction}

Misbehaviour detection in vehicular data has attracted significant interest in recent years. Nevertheless, most of the proposed approaches use centralized Machine Learning (ML), applied to massive amounts of data from different vehicles \cite{van2018survey}. %, that are the clients in these scenarios. 
This approach requires all the data produced by the vehicles in the network to be clustered in one huge data centre, which not only produces a delay in the entire process but also leads to privacy issues as driver and passenger data can be shared. Some works \cite{zhang2021survey, lyu2020threats, aledhari2020federated} state the importance of protecting the clients' personal information, and the need of finding new methods that ensure it. In that sense, traditional centralized machine learning is unable to support such ubiquitous deployments and applications due to infrastructure shortcomings such as limited communication bandwidth, intermittent network connectivity, and strict delay constraints \cite{lyu2020threats}. These problems have made researchers move toward more decentralized learning frameworks \cite{billah2022systematic}, such as Federated learning (FL). FL was proposed by Google \cite{mcmahan2017communication} as a solution to the previous problems. FL is a type of collaborative machine learning where instead of sending the data to a central server, the different clients train a common model and only send the weights created during the training phase to that server. This way, their personal information is protected because the clients use their data to train a model, and benefit from the training of other clients without sharing any information about their dataset. The server aggregates all the weights using what is called an aggregation function and sends the result to the clients so that they continue their training using the updated information. The aggregation function is responsible for summarising the clients’ weights in the server into new ones that will be sent back to the clients. A commonly used aggregation function is FedAvg \cite{mcmahan2017communication}, which computes the average of the weights. Nevertheless, in real case scenarios, as our case, the dataset distributions are not independent and identically distributed (non-IID), which causes a deterioration in the performance of FedAvg \cite{campos2021evaluating}. For this reason, we have implemented in our work a more robust aggregation function against the previous scenarios called Fed+ (or Fedplus) \cite{yu2020fed+}, which is designed to handle non-IID data distributions since it removes the condition that all parties have to converge to a single central point. 

The current state of the art for detecting anomalies or misbehaviour is based on supervised learning \cite{uprety2021privacy,boualouache2022federated,boualouache2022survey}, e.g., classifiers and regressors. Supervised techniques need labelled datasets in order to train the model. However, the labelling of the samples is a very resource-intensive and time-consuming process. Usually the labelling can only be done manually \cite{karoly2018unsupervised} and sometimes is not even possible. Supervised algorithms require this intervention to create the labels of the input and set the output \cite{saravanan2018state}, and also require the training process to have numerous labelled examples to achieve a proper generalization. This leads to a need for a huge computation time for model training. These inconveniences related to the use of labelled data have led to a groundswell of interest in leveraging unsupervised ML methods that utilise unlabeled data \cite{usama2019unsupervised}. Unsupervised learning is used to extract meaningful information on the structure and hierarchies in the data, relying only on the data samples without the need for ground truth files. The extracted knowledge representation can be used as a basis for a deep model that requires fewer labelled examples, as it already has a good understanding of the hidden nature of the data and should be only fine-tuned for the specific task \cite{karoly2018unsupervised}. All these reasons motivate us to implement unsupervised learning in federated scenarios.


%These reasons motivate us for applying unsupervised learning techniques, which in the context of federate learning has great synergy since some types of techniques need less data in order to perform great results \cite{andresini2021autoencoder,cheng2018deep}. Hence, as data is spread through several clients, it does not need that each client holds a huge amount of data.   

%does not need labelled data. Although supervised algorithms are simpler than unsupervised ones, unsupervised learning can see patterns which in other ways could be difficult to realise. 

%We proposed our work in the context of Vehicular Ad Hoc Networks (VANETs). VANETs applications are based on the frequent exchange of safety messages by vehicles which provides traffic safety and efficiency \cite{ghosh2009distributed}. It also enables route planning, road safety and e-commerce applications \cite{grover2011machine}. VANETs networks have a short life expectancy, since the network topology changes very frequently, as nodes are in constant movement,  it is frequent that vehicles are out of range of each other. Furthermore, the density of the network changes over time, e.g., during rush hours \cite{ruj2011data}. Hence, ensuring their security is an essential part, since an attacker could broadcast wrong location information to create fake traffic jams, false alerts, or ghost vehicles \cite{so2018integrating}.

Our work proposes a combination of clustering techniques and a special case of neural networks called autoencoders for misbehaviour detection. %, which can detect anomalous samples without the data has to be labelled during the training. Clustering techniques are utilised for finding anomalies in unlabeled data. 
Clustering algorithms aim to separate the given unlabelled data into clusters that achieve high inner similarity and outer dissimilarity, without relying on signatures or explicit descriptions of attack classes. %, or labelled data for training. 
%Clustering has attracted interest from researchers in the field of intrusion detection since they allow finding anomalies in unlabeled data without explicit labels \cite{syarif2012unsupervised}. 
In particular, we choose Gaussian mixture models (GMM) as clustering technique since it adds probabilities therefore removing the restriction that one point has to belong only to one cluster. Additionally, GMM-based clustering also performs better in several scenarios where other clustering methods are bound to fail \cite{vashishth2019gmmr}. As mentioned, we use autoencoders, in particular Variational Autoencoders (VAE). The main goal of an autoencoder is to reconstruct the input data passed to the neural network. Since they achieve great success in generating abstract features of high-dimensional data, the detection of abnormal samples increases significantly \cite{said2020network}. %A very important fact is that, as a neural network, autoencoders generate weights during their training part, which can be used in FL. Also, as explained before, autoencoders are lighter and need fewer training samples than others neural networks such as Multi-Layer Perceptons \cite{ramchoun2016multilayer}. 
This combination of these unsupervised approaches such as neural networks and clustering techniques has been reported to be more efficient in anomaly detection \cite{aneetha2012combined}. Additionally, we implement Restricted Boltzmann Machines (RBM), a type of neural network which creates adequate initial weights for the VAE, assuring that no client will get stuck in their training. This method, to the best of our knowledge, has not been used before. We provide a comparison between the performance of the variational and the regular autoencoder (AE). Our contributions can be summarised as follows:

%Our method works as follows. First, with GMM we divide the clients’ benign dataset into a certain number of groups depending on certain parameters of the GMM, and cluster these clients based on these parameters chosen in their respective GMM. Next, for each cluster, we make a federated environment where the trained model is a combination of GMM and variational autoencoders (VAE), which are a type of autoencoder that mixes probabilities and neural networks. Additionally, we implement Restricted Boltzmann Machines (RBM), a type of neural network which creates adequate initial weights for the VAE, assuring that no client will get stuck in their training. This method, to the best of our knowledge, has not been used before. We also provide a comparison between the performance of the variational and the simple autoencoder (SAE). Our contributions can be summarised as follows:

\begin{itemize}
    \item Creation of a realistic unsupervised misbehaviour detection scenario which implements GMM and VAE using a more sophisticated aggregation function in order to overcome non-iid scenarios.
    %\item Reduction of bandwidth communication by clustering the clients by their number of GMM components.
    \item Solving convergence problem of FL related to the use of autoencoders by the application of RBMs.
    \item Improving of results comparing to supervised and unsupervised works using our dataset.

\end{itemize}


The structure of the paper it is as follows:
Section \ref{sec:Preeliminaries} provides a explanation of the concepts used in this paper. Section \ref{sec:Related} analyse other works which use GMM and autoencoders, and autoencoders with FL. Then, in \ref{sec:System} we give a deep description of our misbehavior detection system. Section \ref{sec:Evaluation} describes the results of our solution and compare with other methods, and Section \ref{sec:Conlutions} concludes the paper.

==> introduction3.tex <==
\section{Introduction}\label{sec:Introduction}
The application of Machine Learning (ML) techniques for cyberattack detection has attracted significant interest in recent years \cite{ahmad2021network}. However, most of the proposed approaches are based on centralized deployments, which are intended to manage massive amounts of data from different sources. Therefore, all the data produced by such sources is typically shared through a data center. This scenario sets out several issues related to the delay associated with the centralized reasoning process that is usually carried out in the cloud, as well as privacy concerns, especially in the case of sensitive data. Indeed, recent works \cite{zhang2021survey, lyu2020threats, aledhari2020federated} state the importance of protecting clients' personal information, and the need to develop distributed ML approaches to cope with the problems of centralized systems in terms of limited communication bandwidth, intermittent network connectivity, and strict delay constraints \cite{lyu2020threats}. These aspects have motivated researchers to move toward more decentralized ML learning frameworks \cite{billah2022systematic}. In this direction, Federated learning (FL) was proposed \cite{mcmahan2017communication} as a collaborative ML approach where the different data sources (or clients) train a common model, which is updated through an aggregator entity. Therefore, data is not communicated to any external entity and clients benefit from the training of other clients without sharing any information about their dataset. The server aggregates all the weights using an aggregation function and sends the result to the clients so that they continue their training using the updated information. \textcolor{red}{In our system the server is a cloud network. This cloud network will serve as a centralized hub for refining and updating misbehavior detection models by the aggregation of the data process by the clients. By using a cloud-based server, the system can easily scale to accommodate a growing fleet of autonomous vehicles, making it a practical solution for large deployments, and  provide real-time monitoring and analysis of data and model performance across the entire set of clients. Furthermore, related to the pirvacy, integrating federated learning with a public cloud network, the system can add an extra layer of security by anonymizing the data further.  }

An example of a cybersecurity problem that has recently gained significant interest is the well-known \textit{misbehavior detection} in vehicular environments which usually refers to the detection of vehicles transmitting false information that cannot be detected by typical cryptographic mechanisms \cite{van2018survey}. However, the current state of the art for misbehavior detection is usually based on supervised learning techniques \cite{uprety2021privacy,boualouache2022federated,boualouache2022survey} that need labelled datasets to train a model. This process might require human intervention becoming a very resource-intensive and time-consuming activity to have numerous labelled examples in order to achieve a proper generalization \cite{karoly2018unsupervised}, \cite{saravanan2018state}. In the case of vehicular environments, the creation of such labelled dataset could be infeasible due to the impossibility to reproduce a real scenario. Furthermore, supervised learning techniques are not appropriate to detect zero-day attacks, which refer to previously unknown threats. Instead, the use of unsupervised learning techniques could be used to mitigate such concerns \cite{usama2019unsupervised}. In particular, unsupervised learning is used to extract information on the data’s structure and hierarchy by using the data samples without the need for ground truth files. The extracted knowledge representation can be used as a basis for a deep model that requires fewer labelled examples \cite{karoly2018unsupervised}. 

In spite of the advantages provided by unsupervised learning, we notice that most of the proposed approaches for misbehavior detection are based on supervised techniques using unrealistic data distributions considering an FL setting \cite{boualouache2022survey}. Indeed, some of the recent works \cite{uprety2021privacy} are based on artificial divisions of vehicular misbehavior datasets, such as the Vehicular Reference Misbehavior (VeReMi) dataset \cite{van2018veremi}. To fill this gap, our work proposes a combination of clustering techniques and autoencoders (AE) for misbehaviour detection.  On the one hand, clustering algorithms use unlabelled data to create clusters that achieve high inner similarity and outer dissimilarity, without relying on signatures or explicit descriptions of attack classes. In particular, we choose Gaussian mixture models (GMM) as clustering technique since it adds probabilities, therefore, removing the restriction that one point has to belong only to one cluster. Additionally, GMM-based clustering also performs better in several scenarios where other clustering methods do not provide suitable results \cite{vashishth2019gmmr}. On the other hand, we use a specific type of AE called Variational Autoencoder (VAE) \cite{bishop1994neural}. The main goal of an AE is to reconstruct the input data and the variational version is based on a stochastic encoder to map the input to a probability distribution. Since they achieve great success in generating abstract features of high-dimensional data, the detection of abnormal samples increases significantly \cite{said2020network}. Additionally, we implement Restricted Boltzmann Machines (RBM), which represent a type of neural network (NN) used as pre-training layer for the VAE to foster convergence during the federated training process. To the best of our knowledge, this is the first work exploring the use of such techniques in the scope of vehicular misbehavior detection. Furthermore, we use the VeReMi dataset for evaluation purposes by considering a realistic FL setting where each vehicle is intended to train with its local data. We carry out an exhaustive comparison between regular AE and VAE, and unlike most existing FL-enabled misbehavior detection approaches, we use Fed+ \cite{yu2020fed+} as the aggregation function to deal with non-iid scenarios \cite{campos2021evaluating}. Our contributions are summarised as follows:

\begin{itemize}
    \item Unsupervised FL approach based on VAE and GMM considering a realistic partition of the VeReMi dataset for misbehavior detection.
    \item Use of RBMs to enhance the convergence of VAEs in the FL setting.
    \item Application of Fed+ as aggregation function to improve the effectiveness of the approach in the presence of non-iid data distributions.
    \item Comprehensive evaluation to demonstrate the effectiveness of the proposed approach and comparison with recent works using the VeReMi dataset.
\end{itemize}

The structure of the paper is as follows: Section \ref{sec:Preeliminaries} describes the main concepts and techniques used in our work. Section \ref{sec:Related} analyses other works related to the application of GMM and AEs, as well as the use of AEs considering FL settings. Then, in \ref{sec:System} we provide a detailed description of our misbehavior detection system. Section \ref{sec:Evaluation} describes the results of our proposed approach and compares it with recent works using the same dataset. Finally, Section \ref{sec:Conlutions} concludes the paper.

==> preliminaries2.tex <==
\section{Preliminaries}\label{sec:Preeliminaries}
In this section, we describe the main operation of FL, as well as the ML models we used in our approach, including GMM, and VAE. %We will also describe RBMs that improve autoencoders' performance and have a synergy with federated learning.

\subsection{Federated learning (FL)}
Traditional ML approaches are characterized by centralized deployments where different parties are forced to share their data to be analyzed. Such scenario poses significant issues around the needs of network connectivity, latency, as well as the compliance with existing data protection regulations. To overcome such problems, FL \cite{mcmahan2017communication} was proposed as a decentralised approach to train a ML model ensuring that data are not shared. Indeed, Federated learning (FL) scenarios are usually represented by two main components: the central entity (or server), and the data owners (or clients). The communication between these parts is essential for the correct creation of the model. The key of FL is that clients are intended to create a model in a collaborative way by only training with their local data and sharing the model updates through the server. 

 \begin{figure} [!ht]
	\centering
		\includegraphics[scale=0.2]{Images/Preeliminaries/fl_scheme_ae.pdf}
	\caption{Pictorial description of an FL setting}
	\label{fig:FLscheme}
\end{figure}

A visual description of the FL operation is displayed in Fig. \ref{fig:FLscheme} where (1) clients train the model using their dataset. Next, (2) they send the weights resulting weights from the local training to the server, which uses an aggregation function (3) to update the clients' incoming weights. Finally, (4) the server sends the aggregated weights to the clients, which start again another training round through (1). For aggregating the weights in the server, our approach is not based on the well-known FedAvg function \cite{mcmahan2017communication}, but on the Fed+ \cite{yu2020fed+}, which is able to provide better performance in non-iid scenarios compared to FedAvg \cite{campos2021evaluating}. The main characteristic of Fed+ is that parties are not forced to converge to a single central point, as explained below. Hence, the weights are uploaded following the following equation:
 \begin{equation} \label{eq:Fed+weights}
    W^{k+1} = \theta[W^k - \nu \nabla f_k(W^k)] + (1-\theta)Z^k,
\end{equation}
where $\nu$ is the learning rate, $\theta$ is a constant between 0 and 1 that controls the degree of regularisation, and $Z^k$ is the average of clients' weights. As the new weights are an average of local weights and global weights, this means that each party has different weights does not depend on the fact that all clients converge to the same point.


\subsection{Gaussian mixture models}
A Gaussian mixture model (GMM) is a probabilistic model that assumes all the data points are generated from a mixture of a finite number of Gaussian distributions with unknown parameters. Formally, a GMM of $K$ components is a parametric probability density function represented as a weighted sum of $K$ normal distributions, i.e.:
$$p(x|\mu_1,\dots,\mu_K,\sigma_1,\dots,\sigma_K,\pi_1,\dots,\pi_K)=\sum_K \pi_i \mathcal{N}(\mu_i,\sigma_i)$$

where $\mu_i$ are the means, $\sigma_i$ the variances, $\pi_i$ the proportions weights (which sum one and are positives), and $\mathcal{N}$ is a  Gaussian with specified mean and variance. The purpose of using GMMs is the division of the dataset observations into $K$ groups or clusters. Due to their probabilistic nature, GMMs differ from other clustering methods such as K-means \cite{awasthi2012improved} in the fact that an observation can belong to more than one cluster. More specifically, GMMs estimate the likelihood of every observation belonging to each component, and assign the observation to the most likely one. In our work, we exploit these probabilities to classify samples as anomalous or not anomalous. Additionally, GMMs present other advantages such as adapting to the shape of the clusters, handling missing data, and taking into account the variance of the data. These properties are described in depth in  \cite{reynolds2009gaussian}.


\begin{figure} [!ht]
	\centering
		\includegraphics[scale=0.4]{Images/Preeliminaries/Autoencoder.pdf}
	\caption{AE's pictorial description. It consists of a symmetric fully connected NN where the input is compressed through the encoder to the latent space to be reconstructed by the decoder.}
	\label{fig:autoencoderImage}
\end{figure}

\subsection{Variational autoencoder (VAE) and Restricted Boltmanz Machines (RMB)}
\subsubsection{VAE}
An autoencoder (AE) \cite{bishop1994neural} is a particular case of NN where the input and output dimensions coincide, and its layer structure is symmetric. AEs are used to build models by using unlabelled data; therefore, they are an example of unsupervised learning techniques. An AE consists of an encoder and a decoder, as shown in Fig. \ref{fig:autoencoderImage}. The encoder takes the input data and compresses it through the hidden layers into a lower dimension code, called \textit{latent space} ($Z$). Then, the decoder reconstructs this latent space into its original state, that is, the input data. The main goal of AEs is to create a copy as close as possible to the original data. The difference between the input and output is called reconstruction error, which is usually measured using the Root Mean Square Error (RMSE). In a scenario for misbehavior or attack detection, training the model with only benign data will produce high reconstruction error when attack data is passed. Hence, a threshold is set to decide which samples are benign or could be considered as an attack. 

A Variational AE (VAE) \cite{kingma2013auto} is a type of AE whose encoding distribution is regularized, i.e., it approaches a standar normal (or gaussian)  distribution during the training to ensure that its latent space is able to generate new data \cite{zhang2021federated, yao2019unsupervised, sun2018learning, an2015variational}. The main difference between a VAE and an AE is that the VAE is a stochastic generative model that provides calibrated probabilities, while a simple AE is a deterministic discriminative model without a probabilistic foundation. AEs are not suitable to generate new samples, so that it can cause the decoder to provide misleading results since all the information condensed in the latent space is disorganised. For that reason, the VAE is intended to map the encoder distribution $q(Z|X)$ to a standar normal distribution for providing more order in the latent space. For this purpose, the \textit{reparameterization trick} is carried out. From this distribution $q(Z|X)$, it takes its mean $Z_\mu$ and standard deviation $Z_\sigma$. With these two latent variables, a sample is created to the latent variable $Z$ that is sent to the decoder in order to create the predicted output $\hat{X}$. This method also ensures that the network can be trained using backpropagation.  

\begin{figure} [!ht]
	\centering
		\includegraphics[scale=0.35]{Images/Preeliminaries/Vae.pdf}
	\caption{Pictorial description of a VAE. Similar to the AE, but the latent space is change by three layers to ensure the encoder follows a normal distribution.}
	\label{fig:VAEimage}
\end{figure}

Once the VAE has been described, the loss function has to be set.  The main goal of VAE is to create a copy of an input vector. Hence, the RMSE has to be minimized. At the same time, as said previously, the model distribution needs to be as close as possible to a standard gaussian. For this, the Kullback–Leibler Divergence \cite{joyce2011kullback} (KL-divergence) function is used. This function measures how similar two distributions are. Hence, this difference between the encoder distribution and a standard distribution  using the KL-divergence has to be as close as 0 as possible. Therefore, the loss function of VAE is:

\begin{equation}
    Loss(X,\hat{X}) = Loss_{RMSE}(X,\hat{X}) + KL(q(Z|X),\mathcal{N}(0,1))
\end{equation}

\subsubsection{RBM}

A RBM is a stochastic neural network model with a two-layer structure, symmetric connection and no self-feedback, which has a full connection between layers and no connection within layers. The first layer is called the visible layer and contains the original input, and the second layer is called the hidden layer. Among their applications, we find feature extraction, pattern recognition, dimensionality reduction, data classification, and several others. However, as in \cite{wu2021research,pacheco2018restricted,saravanan2020deep}, we will use the RBM for pre-training the VAE, giving us the initial weights for training, assuring its convergence in this case. This pre-training will be made with the same dataset used by the VAE.

==> related2.tex <==
\section{Related Work}\label{sec:Related}
Even though FL is a relatively novel technique, there exists a plethora of works in supervised misbehaviour detection that use FL. However, unsupervised techniques, such as autoencoders, k-means, or deep belief networks, are still in development in this field. Our technique combines GMM and autoencoders for the purpose of unsupervised misbehaviour detection. This approach is scarce in current literature, and when it is present, it differs from ours as we will explain further. We have divided this section in two parts. First, we describe works that use GMM and autoencoder in a non federated setting. And second, we have gathered works that use autoencoders with FL in an unsupervised manner, whether it is variational or not.

%Furthermore, our technique, which combines GMM and autoencoders, described in \ref{sec:System} is also scarce in current literature and differs from ours. 


\subsection{Combination of GMM and autoencoders without FL}
The combination of GMM and autoencoders is an approach that has not been widely explored so far. A Deep Autoencoding Gaussian Mixture Model (DAGMM) for unsupervised anomaly detection is presented in \cite{zong2018deep}. %Their model utilises a deep autoencoder to generate a low-dimensional representation and reconstruction error for each input data point, which is further fed into a GMM. 
DAGMM consists of a compression network for reducing the dimension of the input samples by a deep autoencoder, and an estimation network which predicts their likelihood/energy in the framework of GMM. First, the deep autoencoder is trained with the data on the compression network. Then, the estimation network is able to make meaningful density estimations.
%the use GMM to classify in different clusters but they did it directly, without histograms.
\cite{an2022ensemble} proposes to use unsupervised ensemble autoencoders connected to the GMM to adapt to multiple domains regardless of the skewness of each domain. In such work,  ensemble autoencoders and GMMs are jointly optimized by transforming the optimization of the objective function into a Lagrangian dual problem. Then, they use the Expectation-Maximization (EM) algorithm, which consists of two parts, the ensemble network and the estimation network. Firstly, they use the autoencoder for input dimensionality reduction, and then the estimation network estimates the sample density and classifies those samples with high density as anomalous samples.
%they uses to phases. First the autoencoder part and then pass it to a ensemble model which uses GMM
% variational
Lastly in \cite{liao2018unified}, the authors propose a unified Unsupervised Gaussian Mixture Variational Autoencoder for outlier detection. The VAE first trains a generative distribution and extracts reconstruction-based features. Then they adopt a deep brief network to estimate the component mixture probabilities of the GMM by the latent distribution and extracted features, which is further used by the GMM to estimate sample densities with the EM algorithm.




\subsection{Federated Learning and Autoencoders}

%In \cite{aouedi2022fluids} they make a simple work with a autoencoder and with the dataset UNSW-NB15 
In this section, we focus on the works which combine federated learning and autoencoders, either variational or regular. 
A federated version of the previously described methodology named DAGMM \cite{zong2018deep} is presented in \cite{chen2019network}. They aimed to enhance their model with the federated learning benefits related to the privacy of data of the clients by making each client share its weights of the autoencoder part. \cite{rey2022federated} investigates the possibilities enabled by FL concerning IoT malware detection and studies security issues inherent to this new learning paradigm. In such work, they use both supervised and unsupervised learning.  For the unsupervised method they use autoencoders for detecting anomalies as usual. That is, training the model with benign data and then classifying those samples with high reconstruction error as malign data.
Other works such us \cite{preuveneers2018chained, cetin2019federated, alazzam2022federated} also incorporate autoencoders in its federated environment but in other contexts, such as blockchain and wireless networks. All of them, as in the previous work, detect the anomalies by those which surpass the reconstruction error.

In \cite{wu2022fl}, an anomaly detection classification model that incorporates federated learning and mixed Gaussian variational self-encoding networks named MGVN is proposed. The MGVN network model first constructs a variational self-encoder using a mixed Gaussian prior to extract features from the input data, and then it constructs a deep support vector network with the mixed Gaussian variational self-encoder to compress the feature space. They used a convolutional autoencoder whose encoder part is obtained through the mixed Gaussian variational self-encoder, then the anomalous traffic is detected by using a threshold.

Comparing the works of both sections with ours. The usual way the other authors combine the GMM and autoencoders is by applying first the autoencoder and then passing the results to the GMM. However, we first apply the GMM and transform the data before passing it to the autoencoder as in \cite{zolotukhin2016increasing, garcia2021distributed}, as will be explained in the following section. We benefit equally from the properties of both GMM and VAE. This method enables in our case to classify directly a set of samples and focus on the most challenging ones. Altering any part algorithm will harm the final performance. In \cite{wu2022fl}, they also start applying the GMM part, but they do not transform the autoencoder's input data.


==> system2.tex <==
\section{Proposed misbehavior detection system}\label{sec:System}
This section provides a detailed description about our unsupervised FL-enabled misbehavior detection approach. Furthermore, we describe the dataset used  

\subsection{Dataset and preprocessing} \label{dataandprep}
For evaluation purposes, we use the VeReMi dataset \cite{van2018veremi}, which is a simulated dataset that was created using VEINS and the Luxembourg SUMO Traffic (LuST) scenario \cite{7385539}. LuST is a traffic simulation scenario validated with real driving data. VeReMi utilizes a subsection of the LuST scenario. VeReMi dataset was created by simulating 225 scenarios considering 5 position forging attacks, 3 vehicle densities (low, medium and high), 3 attacker densities (10, 20 and 30 percent), and each parameter set was repeated 5 times for randomization. Finally, the dataset contains the log messages of 498 vehicles. Each file maintains a record of Basic Safety Messages (BSMs) received by a single vehicle (same ID) from neighbouring vehicles (300-meter range) during its entire journey. The files are converted to CSV format differentiating between benign and attack samples. %labeling the type of attack, which are reflected in table \ref{tab:veremi_attacks}, being type 0 benign traffic

Furthermore, we carry out a pre-processing of the VeReMi dataset to deal with the impact of non-iid data distributions on the effectiveness of the misbehavior detection approach. The main reason is that our approach (unlike other recent works, such as \cite{moulahi2022privacy}) considers each vehicle as an FL client using its own data during the federated training process. Indeed, as shown in our previous works \cite{campos2021evaluating}, non-iid data distributions might have a dramatic impact on the effectiveness of the FL-enabled system. For this purpose, we use SMOTE-Tomek \cite{batista2003balancing}, which represents a combination of oversampling and undersampling techniques to balance the class ratio. The new samples in the dataset are created through SMOTE by making linear combinations between close points of the less represented class. Then, Tomek Links is in charge of removing neighbour points that belong to different classes in order to make the classes more differentiable. Initially, the balance of the clients' dataset is 75\% benign-25\% attack. After applying SMOTE-Tomek, the balance is nearly 50-50 in all clients.

\subsection{Detection system}
\subsubsection{Description of the scenario}
The overall system model of our misbehaviour detection approach consists of several vehicles equipped with a ML module to perform the local training. This module trains a local ML model on each vehicle's data and the messages among themselves and the received ones by other vehicles by BSM messages to update the global model shared by the server node in each training round. In case of detecting a misbehaviour, they can communicate such information to the server, which will store the new data in the database. For the communication with the server, vehicles’ messages go through road ITS stations. First, to communicate with these road ITS stations, wireless links are used and then, the communication between the road ITS stations and the cloud is mostly fixed. Based on the previous description, in this system model, vehicles act as FL clients performing local training by using the VeReMi dataset \cite{so2018integrating} (see Section \ref{sec:Evaluation}) and the global model, which is shared by the server in each training round. The server implements an aggregation method (as described in Section \ref{sec:Preeliminaries}) to aggregate the local results from the FL clients. The resulting aggregated model is sent again to the FL clients to be updated through a new training round. 

\subsubsection{Overview of the system}
A global overview of our system model can be looked at Fig. \ref{fig:systemModel}, where the interaction of all the steps involved is reflected. Our model will consist of 3 phases. Firstly, before applying the FL, the clients train the GMM with their benign dataset, then transform this dataset used into histograms and create the initial weights with the RBMs for training the VAE in the next phase (1). These histograms measure for each sample how many dimensions are inside each group created by the GMM and it is important to the last phase of our method. This step is explained deeply in the next section.  Next is the FL phase, where after the initialization, the clients form a federated environment to train their VAE models using the histograms created previously (2). These two phases are made using only their benign datasets. Finally, the third part is the local misbehaviour detection (3). In this phase, after the FL phase, each client classifies the incoming samples as benign or malign. To achieve this, GMMs, for evaluating whether a point belongs or not to one of the groups created by the GMM, utilise the likelihood function \cite{etz2018introduction}. The classification of the points is based on the value of this function, if they are greater than 1, between 1 and 0, and equal to 0. The samples with a value between 0 and 1, will be transformed into histograms and the VAE will classify them depending on the threshold set. % we have the local misbehaviour detection (part (2)), in which malign samples are detected in each client, they apply the GMM as a first filter to classify the samples. For the rest of samples, with the VAE model trained by FL previously, they classify the remaining samples based on the threshold set and the end of the FL.


\begin{figure*} [!ht]
	\centering
		\includegraphics[scale=0.24]{Images/Detection Model/esqmod.pdf}
	\caption{Pictorial description of our the detection model. There are three phases, the first one (1), is the initialization, where the clients train the GMM and create the histograms subsequently. Also, they use RBM to create the initial weights of the VAE. Then, in (2), clients create a federated environment to train their VAE models. And finally, in (3), the local misbehaviour detection is carried out, where each client classifies the samples as benign or malign using the model trained and the threshold $th$ set.}
	\label{fig:systemModel}
\end{figure*}


\iffalse
\begin{figure*}[!htb]
\centering
  \begin{subfigure}{\columnwidth}
    \includegraphics[width=\linewidth]{esqmod1.pdf}
    \caption{Metrics using the original Veremi dataset with FedAvg (Scenario 1) and Fed+ (Scenario 2)} \label{fig:1a}
  \end{subfigure}%
  \hspace*{\fill}   % maximize separation between the subfigures
  \begin{subfigure}{\columnwidth}
    \includegraphics[width=\columnwidth]{esqmod2.pdf}
    \caption{Metrics using the balanced Veremi dataset with FedAvg (Scenario 3) and Fed+ (Scenario 4)} \label{fig:1b}
  \end{subfigure}%
  \hspace*{\fill}   % maximizeseparation between the subfigures
\caption{Comparison of the different scenarios with the original Veremi dataset and balanced Veremi through SMOTE-Tomek} \label{fig:comparacion_escenarios}
\end{figure*}
\fi

\subsubsection{Model training}
Before classifying the samples, the VAE model has to be trained. First, given a client, we preprocess its dataset as described in subsection \ref{dataandprep}, and we use the 80\% of the benign dataset to train the GMM with the number of components previously optimised using the Silhouette coefficient \cite{rousseeuw1987silhouettes}, which  is a metric used to calculate the performance of a particular clustering by examining how separated and compact the clusters are. This first application of the GMM is only for training, to separate the benign traffic into several groups which will serve as the first step in order to choose which samples are benign and which are malign in the next section.
%In order to make a decision on the range of partitions we wanted to try, we compared the computing time of the different parts of our method that are affected most by the number of components of the GMM in Table  \ref{tab:timeComparison}. As one can anticipate, the table shows exponential growth of time (in seconds) as the number of components increases, joining this with the results of the next section we decided to set 300 as the maximum number of components.
%to classify a new point we calculate the value of its likelihood function \cite{etz2018introduction}. If this value is greater than 1, it means that it belongs to one of the groups created by the GMM, so it is classified as benign. If it is equal to 0, it does not belong to one of the groups of the GMM, so it is classified as anomalous. Nevertheless, the samples whose value is between 0 and 1 could be attacks that can mirror the normal traffic. For these latter that cannot be clearly classified

The process of the training part can be seen in algorithm \ref{alg:train}. Firstly, in phase 1, for each client, the GMM divides the benign dataset $B_n$ as many groups $G_n=(g_n^k)_1^{K_n}$ as components $K_n$ set (line 3). Then, we transform the dataset used applying a technique based on computing histogram vectors  \cite{zolotukhin2016increasing} (line 4), that is used in previous works \cite{garcia2021distributed}. This technique creates a matrix $H_n$ which contains the vectors $h^i = (h^i_1,h^i_2,\dots,h^i_{K_n})$ (line 24), where $K_n$ is the number of groups (equal to the number of GMM components) previously set, and each $h^i_k$ is the number of features of the sample $i$ which are within each group $g^k_n$ divided by the total number of features (line 18), i.e, for each feature $j$ of sample $i$ we check whether the value of this feature is within the dimension $j$ of the cluster $g_n^i$ (lines 15-17) (between the dimension $j$ of the center of this cluster minus the standard deviation and the dimension $j$ of the center plus the standard deviation). The function $Dim_j(x)$ of lines 15 and 16 means to take the coordinate $j$ of the point $x$. This histogram $H$ will be used as the input data for training the VAE, whose input dimension will be the number of components previously chosen.

One of the drawbacks of the AEs is that the weights during the training often get stuck and do not converge if they start in a bad initial state. Hence, in our case, as there are a high number of clients involved in FL, it is probable that several clients can get stuck and consequently harm the federated environment. To prevent this, we use RBMs, a stochastic neural network that Hinton and Salakhutdinov \cite{hinton2006reducing} found that they could use trained RBMs to create a correct initialization state for AEs. Hence, in our case, after the creation of the histograms, the RMBs pre-train the VAE using these histograms in order to get the correct initial weights $W^0_n$ for the VAE (lines 5 and 6).

After this initialization, it is phase 2, where we apply FL to train the VAE models of the clients (line 9). All the clients will train the VAE sharing the weights produced during the training (lines 26-34), as it has been described in section \ref{sec:Preeliminaries}. After this training, we set the threshold as

\begin{equation}\label{eq:RecErr}
    th = mean(RE)+0.01*std(RE)
\end{equation}
where $mean(RE)$ and $std(RE)$ are the mean and standard deviation of the reconstruction error (RE) of the VAE respectively (line 10). We use this formula since it will give us a value close to the 95-percentile.

%A summary of the process is reflected in the algorithm \ref{alg:train}. In the algorithm, the function $theshold$ is the equation \ref{eq:RecErr}, $Dim_j$ correspond to take the $j$th coordinate of a point.
\begin{algorithm}
\caption{Complete training of our VAE model}\label{alg:train}

\KwData{$N$ number of clients, $B_n$ Benign dataset of client $n$, $GMM_n$ gaussian mixture model of client $n$, $VAE_n$ VAE model of client $n$, $rounds$ number of rounds in the federated environment, $threshold$ is the equation \ref{eq:RecErr}, $Fedplus$ is the equation \ref{eq:Fed+weights}, and $\theta$ the Fed+ constant.}
\KwResult{VAE model trained and threshold of each client}
(Phase 1)

\For{ $n \in N$}{
$G_n = GMM_n(B_n)$

$H_n =$ Create histograms($B_n$, $G_n$)

$W^0_n = RBM_n(H_n)$

Set $W^0_n$ to $VAE_n$}

(Phase 2)

$FL(VAE_n,H_n, rounds)$

$th_n = threshold(VAE_n)$ \algorithmicforall{ $n \in N$}\hfill \break

Create histograms($B_n$, $G_n$):

\For{ $i \in B_n$}{
\For{ $g\in G_n$}{
\For{ $j \in features(B_n$)}{
Sup\_bound = $Dim_j(Center_g) + Dim_j(Std_g)$

Inf\_bound = $Dim_j(Center_g) - Dim_j(Std_g)$

\If{$j \in [Inferior\_bound, Superior\_bound]$}{
$h_g^i += \frac{1}{length(features)}$

}%\ENDIF
}
}
$h^i=(h^i_1,\dots, h^i_{length(G_n)})$%\ENDFOR
}%\ENDFOR
\textbf{return: }$H=(h^i)_1^{length(B_n)}$ \hfill \break

FL($VAE_n,H_n, rounds$):\hfill

\For{$r$ in [1,$\dots$, $rounds$]}{
Server sends weights $Z$ (or nothing at round 1) to clients

\For{$n \in N$}{
Train $VAE_n$ with $H_n$ 

\text{Get weights }W^r_n\text{ of }VAE_n

W_n^{r+1} = FedPlus(Z, W_n^r, \theta)

Client_n\text{ sends }$W_n$\text{ to server }
}%\ENDFOR \hfill \break
\text{Server aggregates all the }$(W_n)_1^N$\text{ into }$Z$.
}%\ENDFOR
\textbf{return: } $(VAE_n)_1^N$ trained
\end{algorithm}





\subsubsection{Classifying the samples}
In this part of the method, the dataset used contains benign and malign data. In order to classify the samples as benign or malign, as can be seen in Algorithm \ref{alg:cap}, we make use of the likelihood function associated with the GMM (line 37).  Given a sample, we calculate the value of the likelihood function for this point. If this value is greater than 1 (line 38), it means that it belongs to one of the groups created by the GMM, so it is classified as benign (line 39). If it is equal to 0 (line 40), it does not belong to one of the groups of the GMM, so it is classified as anomalous (line 41). Nevertheless, the samples whose value is between 0 and 1 (line 41) could be attacks that can mirror the normal traffic \cite{zolotukhin2016increasing}. For these latter that cannot be directly classified  we transform them into histograms (line 44) previously described and apply the VAE trained in the previous phase (line 45). If the reconstruction error is higher than the threshold (line 46), it means that it is anomalous (line 47), otherwise, it is benign data (line 48). The testing part of our model will be performed by the 20\% of the benign dataset not taken in the training part, with a sample of the same size of malign data.


\begin{algorithm}
\caption{Our misbehaviour detection system}\label{alg:cap}

\KwData{$D_n$ Testing dataset of client $n$, $LF_{GMM_n}$ likelihood function of  gaussian mixture model of client $n$ $GMM_n$, $G_n$ groups created by $GMM_n$, $VAE_n$ VAE model of client $n$, $RMSE$ is the Root Mean Square Error, $th_n$ threshold set by the client $n$}
\KwResult{  Accuracy of the model $a$} \\
\For{$x\in D_n$}{
$p = LF_{GMM_n}(x)$

\eIf{$p\geq 1$}{
$x$ is benign

{\If{$p= 0$}{
$x$ is anomalous}
{$H=Histogram(x, G_n)$ %else

$\hat{H}= VAE_n(H)$

$RE_n(\Hat{H})= RMSE(H, \hat{H})$ 

\eIf{$RE_n(\hat{H}) > th_n$}{
$x$ is anomalous}{
$x$ is benign}
}%\ENDIF
}%\ENDIF
}
}%\ENDFOR \\
Calculate confusion matrix $M$ and get accuracy.\hfill \break

$Histogram(x, G_n):$
\For{$g\in G_n$}{
\For{$j \in features(x$)}{
Sup\_bound = $Dim_j(Center_g) + Dim_j(Std_g)$

Inf\_bound = $Dim_j(Center_g) - Dim_j(Std_g)$ 

\If{ $j \in [Inf\_bound, Sup\_bound]$}{
$h_g^i += \frac{1}{length(features)}$
}%\ENDIF
}
}
\textbf{return: }$h^i=(h^i_1,\dots, h^i_{length(G_n)})$

\end{algorithm}



==> system3.tex <==
\section{Proposed misbehavior detection system}\label{sec:System}
This section provides a detailed description about our unsupervised FL-enabled misbehavior detection approach. Furthermore, we describe the dataset used and how it is preprocessed below. 

\subsection{Dataset and preprocessing} \label{dataandprep}
For evaluation purposes, we use the VeReMi dataset \cite{van2018veremi}, which is a simulated dataset that was created using VEINS and the Luxembourg SUMO Traffic (LuST) scenario \cite{7385539}. LuST is a traffic simulation scenario validated with real driving data. VeReMi utilizes a subsection of the LuST scenario. VeReMi dataset was created by simulating 225 scenarios considering 5 position forging attacks, 3 vehicle densities (low, medium and high), and 3 attacker densities (10, 20 and 30 percent), and each parameter set was repeated 5 times for randomization. Finally, the dataset contains the log messages of 498 vehicles. Each file maintains a record of Basic Safety Messages (BSMs) received by a single vehicle (same ID) from neighbouring vehicles (300-meter range) during its entire journey. The files are converted to CSV format differentiating between benign and attack samples. %labeling the type of attack, which are reflected in table \ref{tab:veremi_attacks}, being type 0 benign traffic

Furthermore, we carry out a pre-processing of the VeReMi dataset to deal with the impact of non-iid data distributions on the effectiveness of the misbehavior detection approach. The main reason is that our approach (unlike other recent works, such as \cite{moulahi2022privacy}) considers each vehicle as an FL client using its own data during the federated training process. Indeed, as shown in our previous works \cite{campos2021evaluating}, non-iid data distributions might have a dramatic impact on the effectiveness of the FL-enabled system. For this purpose, we use SMOTE-Tomek \cite{batista2003balancing}, which represents a combination of oversampling and undersampling techniques to balance the class ratio. The new samples in the dataset are created through SMOTE by making linear combinations between close points of the less-represented class. Then, Tomek Links is in charge of removing neighbour points that belong to different classes in order to make the classes more differentiable. Initially, the balance of the clients' dataset is 75\% benign-25\% attack. After applying SMOTE-Tomek, the balance is nearly 50-50 in all clients.

\subsection{System description}
After describing the dataset and the pre-processing we carry out, below we provide a detailed explanation of the proposed system, including the different phases of the misbehavior detection approach. 

\subsubsection{Overview}
A global overview of our system is shown in Fig. \ref{fig:systemModel}, which includes the relationship between the different components and techniques previously described. As already mentioned, vehicles act as FL clients performing local training by using the VeReMi dataset and the global model that is updated in each training round. In particular, our approach consists of 3 phases. Firstly, during Phase 1 (Initialization), clients train the GMM with their benign dataset. Then, this data is transformed into histograms that are used to create the initial weights for training the VAE by using the RBMs. For each sample, these histograms measure which features are within each group created by the GMM. Once each client has initialized its corresponding VAE, Phase 2 (Federated learning) is carried out by following the steps described in Section \ref{sec:Preeliminaries}, so that each client performs a local training by using its own data in each training round. The server implements an aggregation method to aggregate the local results from the FL clients, and the resulting aggregated model is sent again to the FL clients to be updated through a new training round. In Phase 3 (Local misbehavior detection), after the federated training process is finished, each client has a trained VAE to be used for classification purposes in order to detect potential misbehavior. In particular, the GMM's likelihood function \cite{etz2018introduction} is used to evaluate whether a point belongs or not to one of the groups previously created in Phase 1. Depending on the likelihood value, the sample is considered a benign sample (greater than 1) or an attack (0). In case of a value between 0 and 1, a histogram is created for that sample, and the local VAE is used to classify it depending on a certain threshold value. These processes are further detailed in the following subsections. 


\begin{figure*} [!ht]
	\centering
		\includegraphics[scale=0.24]{Images/Detection Model/esqmod.pdf}
	\caption{Pictorial description of our misbehavior detection system. There are three phases, the first one (1), is the initialization, where the clients train the GMM and create the histograms subsequently. Also, they use RBM to create VAE's initial weights. Then, in (2), clients create a federated environment to train their VAE models. And finally, in (3), the local misbehaviour detection is carried out, where each client classifies the samples as benign or malign using the model trained and the threshold $th$ set.}
	\label{fig:systemModel}
\end{figure*}


\iffalse
\begin{figure*}[!htb]
\centering
  \begin{subfigure}{\columnwidth}
    \includegraphics[width=\linewidth]{esqmod1.pdf}
    \caption{Metrics using the original Veremi dataset with FedAvg (Scenario 1) and Fed+ (Scenario 2)} \label{fig:1a}
  \end{subfigure}%
  \hspace*{\fill}   % maximize separation between the subfigures
  \begin{subfigure}{\columnwidth}
    \includegraphics[width=\columnwidth]{esqmod2.pdf}
    \caption{Metrics using the balanced Veremi dataset with FedAvg (Scenario 3) and Fed+ (Scenario 4)} \label{fig:1b}
  \end{subfigure}%
  \hspace*{\fill}   % maximizeseparation between the subfigures
\caption{Comparison of the different scenarios with the original Veremi dataset and balanced Veremi through SMOTE-Tomek} \label{fig:comparacion_escenarios}
\end{figure*}
\fi

\subsubsection{Model training}
As previously mentioned, the model training process is split into two main phases: Initialization and Federated learning. Before starting this process, it should be noted that, for each client, we pre-process its corresponding dataset as described in subsection \ref{dataandprep}, and we use the 80\% of the benign dataset to train the GMM with the number of components previously optimised. Toward this end, we use the Silhouette coefficient \cite{rousseeuw1987silhouettes}, which represents a metric to calculate the performance of a particular clustering by examining how separated and compact the clusters are. 

The model training process is further detailed in Algorithm \ref{alg:train}. Firstly, in Phase 1, for each client, GMM is used to divide the benign dataset $B_n$ as many groups $G_n=(g_n^k)_1^{K_n}$ as components $K_n$ are previously computed (line 3). Then, the data is transformed into histogram vectors  \cite{zolotukhin2016increasing} (line 4), which are used in our previous works \cite{garcia2021distributed}. This technique creates a matrix $H_n$ containing the vectors $h^i = (h^i_1,h^i_2,\dots,h^i_{K_n})$ (line 24), where $K_n$ is the number of groups (equal to the number of GMM components), and each $h^i_k$ is the number of features of sample $i$ that are within each group $g^k_n$ divided by the total number of features (line 18). Therefore, for each feature $j$ of sample $i$ we check whether the value of this feature is within the dimension $j$ of the cluster $g_n^i$ (lines 15-17)\footnote{That is, between the dimension $j$ of the center of this cluster minus the standard deviation and the dimension $j$ of the center plus the standard deviation}. Furthermore, it should be noted that function $Dim_j(x)$ is only intended to take the coordinate $j$ of point $x$. The resulting histogram $H$ is used by the RBM to pre-train the VAE in order to get the initial weights $W^0_n$ (lines 5-6) for the next steps. 

In Phase 2, the FL process is carried out by the different clients using the local VAE models (line 9), whose input dimension is the number of components previously set. Each client is intended to train locally its corresponding VAE model and share the resulting weights in each training round (lines 26-34), as previously described in Section \ref{sec:Preeliminaries}. Once this process is complete after a certain number of rounds, we set the threshold as:

\begin{equation}\label{eq:RecErr}
    th = mean(RE)+0.01*std(RE)
\end{equation}
where $mean(RE)$ and $std(RE)$ are the mean and standard deviation of the VAE's reconstruction error (RE) respectively (line 10). We use this formula since it provides a value close to the 95-percentile.

%A summary of the process is reflected in the algorithm \ref{alg:train}. In the algorithm, the function $theshold$ is the equation \ref{eq:RecErr}, $Dim_j$ correspond to take the $j$th coordinate of a point.
\begin{algorithm}
\caption{Model training}\label{alg:train}

\KwData{$N$ set of clients, $B_n$ benign dataset of client $n$, $GMM_n$ gaussian mixture model of client $n$, $VAE_n$ VAE model of client $n$, $rounds$ number of rounds in the federated environment, $threshold$ is the equation \ref{eq:RecErr}, $Fedplus$ is the equation \ref{eq:Fed+weights}, and $\theta$ the Fed+ constant.}
\KwResult{VAE model trained and threshold of each client}
(Phase 1)

\For{ $n \in N$}{
$G_n = GMM_n(B_n)$

$H_n =$ Create histograms($B_n$, $G_n$)

$W^0_n = RBM_n(H_n)$

Set $W^0_n$ to $VAE_n$}

(Phase 2)

$FL(VAE_n,H_n, rounds)$

$th_n = threshold(VAE_n)$ \algorithmicforall{ $n \in N$}\hfill \break

Create histograms($B_n$, $G_n$):

\For{ $i \in B_n$}{
\For{ $g\in G_n$}{
\For{ $j \in features(B_n$)}{
Sup\_bound = $Dim_j(Center_g) + Dim_j(Std_g)$

Inf\_bound = $Dim_j(Center_g) - Dim_j(Std_g)$

\If{$j \in [Inf\_bound, Sup\_bound]$}{
$h_g^i += \frac{1}{length(features)}$

}%\ENDIF
}
}
$h^i=(h^i_1,\dots, h^i_{length(G_n)})$%\ENDFOR
}%\ENDFOR
\textbf{return: }$H=(h^i)_1^{length(B_n)}$ \hfill \break

FL($VAE_n,H_n, rounds$):\hfill

\For{$r$ in [1,$\dots$, $rounds$]}{
If $r>1$ server sends mean weights $Z$ to clients,\hfill \\otherwise 0 
%\If{$r>1$}{Server sends mean weights $Z$ to clients}
%Server sends weights $Z$ (or nothing at round 1) to clients

\For{$n \in N$}{
Train $VAE_n$ with $H_n$ 

\text{Get weights }W^r_n\text{ of }VAE_n

W_n^{r+1} = FedPlus(Z, W_n^r, \theta)

Client_n\text{ sends }$W_n$\text{ to server }
}%\ENDFOR \hfill \break
\text{Server aggregates all the }$(W_n)_1^N$\text{ into }$Z$.
}%\ENDFOR
\textbf{return: } $(VAE_n)_1^N$ trained
\end{algorithm}


\subsubsection{Local misbehavior detection}
After the previous steps are complete, each vehicle is equipped with a model to detect potential misbehavior detection (Phase 3 in Figure \ref{fig:systemModel}) based on the classification of samples during the testing process of the model. For this purpose, each vehicle employs the portion of benign data that was not used for training (i.e., 20\%), as well as the same size of attack data. The process is detailed in Algorithm \ref{alg:cap}, which is based on the calculation of the likelihood function associated with the GMM (line 38) for each sample of a vehicle's testing dataset. If this value is greater than or equal to 1 (line 39), it means that such sample belongs to one of the groups created by the GMM, so it is classified as benign (line 40). If it is equal to 0 (line 42), it does not belong to a GMM group, so it is classified as anomalous (line 43). Then, the samples whose value is between 0 and 1 (line 44) could represent attacks mirroring normal traffic \cite{zolotukhin2016increasing}. These samples are transformed into histograms (line 45) as previously described. Then, the VAE that was trained in the previous phase is applied (line 46); if the reconstruction error is higher than the threshold (line 47), it means that it is anomalous (line 49), otherwise, such sample is considered as benign data (line 51). 


\begin{algorithm}
\caption{Local misbehavior detection}\label{alg:cap}

\KwData{$D_n$ Testing dataset of client $n$, $LF_{GMM_n}$ likelihood function of  gaussian mixture model of client $n$ $GMM_n$, $G_n$ groups created by $GMM_n$, $VAE_n$ VAE model of client $n$, $RMSE$ is the Root Mean Square Error, $th_n$ threshold set by the client $n$}
\KwResult{  Accuracy of the model $a$} \\
\For{$x\in D_n$}{
$p = LF_{GMM_n}(x)$

\eIf{$p\geq 1$}{
$x$ is benign

}{\eIf{$p= 0$}{
$x$ is anomalous}{
{$H=Histogram(x, G_n)$ %else

$\hat{H}= VAE_n(H)$

$RE_n(\Hat{H})= RMSE(H, \hat{H})$ 

\eIf{$RE_n(\hat{H}) > th_n$}{
$x$ is anomalous}{
$x$ is benign}
}%\ENDIF
}
}%\ENDIF
}
%\ENDFOR \\
Calculate confusion matrix $M$ and get accuracy.\hfill \break

$Histogram(x, G_n):$
\For{$g\in G_n$}{
\For{$j \in features(x$)}{
Sup\_bound = $Dim_j(Center_g) + Dim_j(Std_g)$

Inf\_bound = $Dim_j(Center_g) - Dim_j(Std_g)$ 

\If{ $j \in [Inf\_bound, Sup\_bound]$}{
$h_g^i += \frac{1}{length(features)}$
}%\ENDIF
}
}
\textbf{return: }$h^i=(h^i_1,\dots, h^i_{length(G_n)})$

\end{algorithm}



==> system4.tex <==
\section{Proposed misbehavior detection system}\label{sec:System}
This section provides a detailed description about our unsupervised FL-enabled misbehavior detection approach. Furthermore, we describe the dataset used and how it is preprocessed below. 

\subsection{Dataset and preprocessing} \label{dataandprep}
For evaluation purposes, we use the VeReMi \cite{van2018veremi} and VeReMi extension \cite{kamel2020veremi} datasets. On one hand, VeReMi is a simulated dataset that was created using VEINS and the Luxembourg SUMO Traffic (LuST) scenario \cite{7385539}. On the other hand, VeReMi extension make use of Framework For Misbehavior Detection (F²MD). F²MD is a VEINS extension that enables the recreation and detection of various misbehavior detection use cases. LuST is a traffic simulation scenario validated with real driving data. VeReMi utilizes a subsection of the LuST scenario. VeReMi dataset was created by simulating 225 scenarios considering 5 position forging attacks, 3 vehicle densities (low, medium and high), and 3 attacker densities (10, 20 and 30 percent), and each parameter set was repeated 5 times for randomization. Finally, the dataset contains the log messages of 498 vehicles. For VeReMi extension, it uses subsection of the LuST
network with a size 1.61 \textit{km²} and a peak density of 67.4 \textit{Veh/km²}. Furthermore, VeReMi extension contain two vehicle densities, one in the rush hour time (7h-9h), and another in low traffic time (14h-16h). Each file maintains a record of Basic Safety Messages (BSMs) received by a single vehicle (same ID) from neighbouring vehicles (300-meter range) during its entire journey. The files are converted to CSV format differentiating between benign and attack samples. %labeling the type of attack, which are reflected in table \ref{tab:veremi_attacks}, being type 0 benign traffic

Furthermore, we carry out a pre-processing of the VeReMi dataset to deal with the impact of non-iid data distributions on the effectiveness of the misbehavior detection approach. The main reason is that our approach (unlike other recent works, such as \cite{moulahi2022privacy}) considers each vehicle as an FL client using its own data during the federated training process. Indeed, as shown in our previous works \cite{campos2021evaluating}, non-iid data distributions might have a dramatic impact on the effectiveness of the FL-enabled system. For this purpose, we use SMOTE-Tomek \cite{batista2003balancing}, which represents a combination of oversampling and undersampling techniques to balance the class ratio. The new samples in the dataset are created through SMOTE by making linear combinations between close points of the less-represented class. Then, Tomek Links is in charge of removing neighbour points that belong to different classes in order to make the classes more differentiable. Initially, the balance of the clients' dataset is 75\% benign-25\% attack. After applying SMOTE-Tomek, the balance is nearly 50-50 in all clients. Finally, as explained in section \ref{sec:Preeliminaries}, GMM are a sum of normal distributions. Therefore, the dataset has to follow a Gaussian distribution. In this sense, we normalise the dataset and check whether it fits to a Gaussian distribution by applying the Shapiro-wilk test \cite{SHAPIRO1965}. After applying the Shapiro-wilk test we have  a Shapiro-wilk score of 0.98 and $p$-value of $0.99>0.05$, meaning that the dataset follows a Gaussian distribution.

\subsection{System description}
After describing the dataset and the pre-processing we carry out, below we provide a detailed explanation of the proposed system, including the different phases of the misbehavior detection approach. 

\subsubsection{Overview}
A global overview of our system is shown in Fig. \ref{fig:systemModel}, which includes the relationship between the different components and techniques previously described. As already mentioned, vehicles act as FL clients performing local training by using the VeReMi dataset and the global model that is updated in each training round. In particular, our approach consists of 3 phases. Firstly, during Phase 1 (Initialization), clients train the GMM with their benign dataset. Then, this data is transformed into histograms that are used to create the initial weights for training the VAE by using the RBMs. For each sample, these histograms measure which features are within each group created by the GMM. Once each client has initialized its corresponding VAE, Phase 2 (Federated learning) is carried out by following the steps described in Section \ref{sec:Preeliminaries}, so that each client performs a local training by using its own data in each training round. The server implements an aggregation method to aggregate the local results from the FL clients, and the resulting aggregated model is sent again to the FL clients to be updated through a new training round. \textcolor{red}{In this part, the clients would be the vahicles and the server the could network. The autonomous vehicles serve as edge devices with on-board computing capabilities. FL is employed to detect cyberattacks locally in these vehicles. The cloud network can then aggregate data from various vehicles and further analyze it to gain a holistic view of the cybersecurity landscape.} In Phase 3 (Local misbehavior detection), after the federated training process is finished, each client has a trained VAE to be used for classification purposes in order to detect potential misbehavior. In particular, the GMM's likelihood function \cite{etz2018introduction} is used to evaluate whether a point belongs or not to one of the groups previously created in Phase 1. Depending on the likelihood value, the sample is considered a benign sample (greater than 1) or an attack (0). In case of a value between 0 and 1, a histogram is created for that sample, and the local VAE is used to classify it depending on a certain threshold value. These processes are further detailed in the following subsections.


\begin{figure*} [!ht]
	\centering
		\includegraphics[width=2\columnwidth]{Images/Detection Model/esqmod_rev.pdf}
	\caption{Pictorial description of our misbehavior detection system. There are three phases, the first one (1), is the initialization, where the clients train the GMM and create the histograms subsequently. Also, they use RBM to create VAE's initial weights. Then, in (2), clients create a federated environment to train their VAE models. And finally, in (3), the local misbehaviour detection is carried out, where each client classifies the samples as benign or malign using the model trained and the threshold $th$ set.}
	\label{fig:systemModel}
\end{figure*}


\iffalse
\begin{figure*}[!htb]
\centering
  \begin{subfigure}{\columnwidth}
    \includegraphics[width=\linewidth]{esqmod1.pdf}
    \caption{Metrics using the original Veremi dataset with FedAvg (Scenario 1) and Fed+ (Scenario 2)} \label{fig:1a}
  \end{subfigure}%
  \hspace*{\fill}   % maximize separation between the subfigures
  \begin{subfigure}{\columnwidth}
    \includegraphics[width=\columnwidth]{esqmod2.pdf}
    \caption{Metrics using the balanced Veremi dataset with FedAvg (Scenario 3) and Fed+ (Scenario 4)} \label{fig:1b}
  \end{subfigure}%
  \hspace*{\fill}   % maximizeseparation between the subfigures
\caption{Comparison of the different scenarios with the original Veremi dataset and balanced Veremi through SMOTE-Tomek} \label{fig:comparacion_escenarios}
\end{figure*}
\fi

\subsubsection{Model training}
As previously mentioned, the model training process is split into two main phases: Initialization and Federated learning. Before starting this process, it should be noted that, for each client, we pre-process its corresponding dataset as described in subsection \ref{dataandprep}, and we use the 80\% of the benign dataset to train the GMM with the number of components previously optimised. Toward this end, we use the Silhouette coefficient \cite{rousseeuw1987silhouettes}, which represents a metric to calculate the performance of a particular clustering by examining how separated and compact the clusters are. 

The model training process is further detailed in Algorithm \ref{alg:train}. Firstly, in Phase 1, for each client, GMM is used to divide the benign dataset $B_n$ as many groups $G_n=(g_n^k)_1^{K_n}$ as components $K_n$ are previously computed (line 2). Then, the data is transformed into histogram vectors  \cite{zolotukhin2016increasing} (line 3), which are used in our previous works \cite{garcia2021distributed}. This technique creates a matrix $H_n$ containing the vectors $h^i = (h^i_1,h^i_2,\dots,h^i_{K_n})$ (line 21), where $K_n$ is the number of groups (equal to the number of GMM components), and each $h^i_k$ is the number of features of sample $i$ that are within each group $g^k_n$ divided by the total number of features (line 15). Therefore, for each feature $j$ of sample $i$ we check whether the value of this feature is within the dimension $j$ of the cluster $g_n^i$ (lines 12-14)\footnote{That is, between the dimension $j$ of the center of this cluster minus the standard deviation and the dimension $j$ of the center plus the standard deviation}. Furthermore, it should be noted that function $Dim_j(x)$ is only intended to take the coordinate $j$ of point $x$. The resulting histogram $H$ is used by the RBM to pre-train the VAE in order to get the initial weights $W^0_n$ (lines 4-5) for the next steps. 

In Phase 2, the FL process is carried out by the different clients using the local VAE models (line 7), whose input dimension is the number of components previously set. Each client is intended to train locally its corresponding VAE model and share the resulting weights in each training round (lines 22-32), as previously described in Section \ref{sec:Preeliminaries}. Once this process is complete after a certain number of rounds, we set the threshold as:


\begin{equation}\label{eq:RecErr}
    th = mean(RE)+0.01*std(RE)
\end{equation}
where $mean(RE)$ and $std(RE)$ are the mean and standard deviation of the VAE's reconstruction error (RE) respectively (line 10). We use this formula since it provides a value close to the 95-percentile.

%A summary of the process is reflected in the algorithm \ref{alg:train}. In the algorithm, the function $theshold$ is the equation \ref{eq:RecErr}, $Dim_j$ correspond to take the $j$th coordinate of a point.
\begin{algorithm}
\caption{Model training}\label{alg:train}
\begin{algorithmic}[1]
\REQUIRE{$N$ set of clients, $B_n$ benign dataset of client $n$, $GMM_n$ gaussian mixture model of client $n$, $VAE_n$ VAE model of client $n$, $rounds$ number of rounds in the federated environment, $threshold$ is the equation \ref{eq:RecErr}, $Fedplus$ is the equation \ref{eq:Fed+weights}, and $\theta$ the Fed+ constant.}
\ENSURE{VAE model trained and threshold of each client}\hfill \break
\textbf{(Phase 1)}
\FOR{$n \in N$}
\STATE $G_n = GMM_n(B_n)$
\STATE $H_n =$ Create histograms($B_n$, $G_n$)
\STATE $ W^0_n = RBM_n(H_n)$
\STATE Set $W^0_n$ to $VAE_n$
\ENDFOR

\vspace{5pt}
\textbf{(Phase 2)}
\STATE $FL(VAE_n,H_n, rounds)$
\STATE $th_n = threshold(VAE_n) \forall n \in N$ 

\vspace{5pt}
Create histograms($B_n$, $G_n$):
\FOR{ $i \in B_n$}
\FOR{$g\in G_n$}
\FOR{$j \in features(B_n$)}
\STATE Sup\_bound = $Dim_j(Center_g) + Dim_j(Std_g)$
\STATE Inf\_bound = $Dim_j(Center_g) - Dim_j(Std_g)$
\IF{$j \in [Inf\_bound, Sup\_bound]$}
\STATE $h_g^i += \frac{1}{length(features)}$
\ENDIF
\ENDFOR
\ENDFOR
\STATE $h^i=(h^i_1,\dots, h^i_{length(G_n)})$
\ENDFOR
\STATE \textbf{return: }$H=(h^i)_1^{length(B_n)}$ \hfill \break

FL($VAE_n,H_n, rounds$):
\FOR{$r$ in [1,$\dots$, $rounds$]}
\IF{$r>1$}
\STATE Server sends mean weights $Z$ to clients, otherwise the clients use $W^0_n$
\ENDIF
\FOR{$n \in N$}
\STATE Train $VAE_n$ with $H_n$ 
\STATE $\text{Get weights }W^r_n\text{ of }VAE_n$
\STATE $W_n^{r+1} = FedPlus(Z, W_n^r, \theta)$
\STATE Client_n\text{ sends }$W_n$\text{ to server }
\ENDFOR
\STATE \text{Server aggregates all the }$(W_n)_1^N$\text{ into }$Z$.
\ENDFOR
\STATE \textbf{return: } $(VAE_n)_1^N$ trained
\end{algorithmic}
\end{algorithm}

\subsubsection{Local misbehavior detection}
After the previous steps are complete, each vehicle is equipped with a model to detect potential misbehavior detection (Phase 3 in Figure \ref{fig:systemModel}) based on the classification of samples during the testing process of the model. For this purpose, each vehicle employs the portion of benign data that was not used for training (i.e., 20\%), as well as the same size of attack data. The process is detailed in Algorithm \ref{alg:cap}, which is based on the calculation of the likelihood function associated with the GMM (line 2) for each sample of a vehicle's testing dataset. If this value is greater than or equal to 1 (line 3), it means that such sample belongs to one of the groups created by the GMM, so it is classified as benign (line 4). If it is equal to 0 (line 5), it does not belong to a GMM group, so it is classified as anomalous (line 6). Then, the samples whose value is between 0 and 1 (line 7) could represent attacks mirroring normal traffic \cite{zolotukhin2016increasing}. These samples are transformed into histograms (line 8) as previously described. Then, the VAE that was trained in the previous phase is applied to reconstruct the histogram (line 9); if the reconstruction error is higher than the threshold (line 11), it means that it is anomalous (line 12), otherwise, such sample is considered as benign data (line 14). 



\begin{algorithm}
\caption{Local misbehavior detection (Phase 3)}\label{alg:cap}

\begin{algorithmic}[1]
\REQUIRE{$D_n$ Testing dataset of client $n$, $LF_{GMM_n}$ likelihood function of  gaussian mixture model of client $n$ $GMM_n$, $G_n$ groups created by $GMM_n$, $VAE_n$ VAE model of client $n$, $RMSE$ is the Root Mean Square Error, $th_n$ threshold set by the client $n$\hfill \break}
\ENSURE{  Accuracy of the model $a$\hfill \break} \\
\FOR{$x\in D_n$}
\STATE $p = LF_{GMM_n}(x)$
\IF{$p\geq 1$}
\STATE $x$ is benign
\ELSIF{$p= 0$}
\STATE $x$ is anomalous
\ELSE
\STATE  $H=Histogram(x, G_n)$%else
\STATE $\hat{H}= VAE_n(H)$
\STATE $RE_n(\Hat{H})= RMSE(H, \hat{H})$ 
\IF{$RE_n(\hat{H}) > th_n$}
\STATE $x$ is anomalous
\ELSE
\STATE $x$ is benign
\ENDIF
\ENDIF
\ENDFOR 
\STATE Calculate confusion matrix $M$ and get accuracy.\hfill \break

$Histogram(x, G_n):$
\FOR{$g\in G_n$}
\FOR{$j \in features(x$)}
\STATE Sup\_bound = $Dim_j(Center_g) + Dim_j(Std_g)$
\STATE Inf\_bound = $Dim_j(Center_g) - Dim_j(Std_g)$ 
\IF{ $j \in [Inf\_bound, Sup\_bound]$}
\STATE $h_g^i += \frac{1}{length(features)}$
\ENDIF
\ENDFOR
\ENDFOR
\STATE \textbf{return: }$h^i=(h^i_1,\dots, h^i_{length(G_n)})$
\end{algorithmic}
\end{algorithm}



